Stay Safe under Panic: Affine Rust Programming with Multiparty Session Types

Communicating systems comprise diverse software components across networks. To ensure their robustness, modern programming languages such as Rust provide both strongly typed channels, whose usage is guaranteed to be affine (at most once), and cancellation operations over binary channels. For coordinating components to correctly communicate and synchronise with each other, we use the structuring mechanism from multiparty session types, extending it with affine communication channels and implicit/explicit cancellation mechanisms. This new typing discipline, affine multiparty session types (AMPST), ensures cancellation termination of multiple, independently running components and guarantees that communication will not get stuck due to error or abrupt termination. Guided by AMPST, we implemented an automated generation tool (MultiCrusty) of Rust APIs associated with cancellation termination algorithms, by which the Rust compiler auto-detects unsafe programs. Our evaluation shows that MultiCrusty provides an efficient mechanism for communication, synchronisation and propagation of the notifications of cancellation for arbitrary processes. We have implemented several usecases, including popular application protocols (OAuth, SMTP), and protocols with exception handling patterns (circuit breaker, distributed logging).

==> Implementation.tex <==
\section{Design and implementation of~\mpstrust}
\label{sec:implementation}

The different processes involved in the same communication in multiparty session types.

\paragraph{\bf Multiparty channels as an ordered tuple of binary channels.}
The main idea of the design of our framework is
that a multiparty session can be realised with two ingredients:
(1) a list of separate binary sessions (one session for each pair of
participants) and (2) a stack that imposes the ordering between the binary channels.
~\Cref{lst:MPSTMeshedChannelsPrimitives} (lines~\ref{line:mpst:beg} --~\ref{line:mpst:end}) shows the
implementation of a multiparty channel in a 3-party protocol. The \CODE{MeshedChannels} structure holds two
fields, \CODE{session1} and \CODE{session2}, that are of a binary session type.
The different elements of code are highlighted as follow: \CODE{functions}, \CODE{macros}, \CODE{types/enums},
\CODE{aliases}, \CODE{primitives} and \CODE{traits}.
For illustration purpose, we show only the implementation of a multiparty channel for three processes.
The same approach can be generalised, using our code generation tool, to any number of communicating processes.
For example, in the case of a
protocol with four roles, each multiparty session will have four fields -- a field for the binary session between
each pair of participants and a field for the stack.

\begin{figure}[t]
	\begin{minipage}[l]{0.9\textwidth}
		\begin{rustlisting}[basicstyle=\scriptsize\ttfamily]
			// Basic structure for MPST
			pub struct MeshedChannels< S1: Session, S2: Session, R: Role, N: Role> {*@ \label{line:mpst:beg} @*
				pub session1: S1, pub session2: S2, pub stack: R, pub name: N
			} *@ \label{line:mpst:end} @*
		\end{rustlisting}
	\end{minipage}
	\begin{minipage}[r]{0.5\textwidth}
		%\begin{rustlisting}[basicstyle=\scriptsize\ttfamily]
		%// Basic Choose/Offer for MPST
		%pub type ChooseMpst<S1, S2> =
		% Send<Either<S1, S2 >, End>;		
		%
		%pub type OfferMpst<S1, S2> =
		% Recv<Either<S1, S2>, End>;
		%\end{rustlisting}
	\end{minipage}
	\begin{minipage}[l]{0.9\textwidth}
		{\lstset{firstnumber=4}
			\begin{rustlisting}[basicstyle=\scriptsize\ttfamily]
				// Implementation of a communication function from the mpst-rust library
				pub fn send_mpst_a_to_b<T, S1, S2, R, N>(x: T, *@ \label{line:mpst:send} @*
				s: MeshedChannels<Send<T, S1>, S2, RoleB<R>>, RoleA<RoleEnd>) -> MeshedChannels<S1, S2, R, RoleA<RoleEnd>>
				where T: std::marker::Send, S1: Session, S2: Session, R: Role, N: Role
					{
						let new_session = send(x, s.session1);
						let new_stack = next_a_to_b(s.stack);
						...
					} *@ \label{line:mpst:close} @*

			\end{rustlisting}}
	\end{minipage}
	\begin{minipage}[l]{0.9\textwidth}
		{\lstset{firstnumber=9}
			\begin{rustlisting}[basicstyle=\scriptsize\ttfamily]
				/// Offer a choice at A from C wrapped in an `enum`
				#[macro_export]
				macro_rules! offer_mpst_a_to_c {($session ... => { *@ \label{line:offer:start} @*
					let (l, s) = recv_mpst_a_to_c($session)?; // receive a label l
					cancel(s); // cancel the existing binary channels on s
					match l { pat_i => invoke...} // Call the associated function *@ \label{line:offer:end} @*
					// with a new MeshedChannels
				}

				#[macro_export]
				macro_rules! choose_mpst_c_to_all($session:expr, $labelone:path, $labeltwo:path) { *@ \label{line:choice:start} @*
					let (channel_1_2, channel_2_1) = <_ as Session>::new();
					let (channel_1_3, channel_3_1) = <_ as Session>::new();
					let (channel_3_2, channel_2_3) = <_ as Session>::new();

					let (stack_1, _) = <_ as Role>::new();

					let (name_1, _) = <RoleA<RoleEnd> as Role>::new();
					let (name_2, _) = <RoleB<RoleEnd> as Role>::new();
					let (name_3, _) = <RoleC<RoleEnd> as Role>::new();

					let s = $session;

					let _ = { // Checks the stack
					fn temp(r: &RoleBroadcast) -> Result<(), Box<dyn std::error::Error>>
						{
							Ok(())
						}
						temp(&s.stack)
					};

					let _ = send($labelone::(
						MeshedChannels {
								session1: channel_1_2,
								session2: channel_1_3,
								stack: stack_1,
								name: name_1
							}),
						s.session1
					);
					let _ = send($labeltwo::(
						MeshedChannels {
								session1: channel_2_1,
								session2: channel_2_3,
								stack: stack_2,
								name: name_2
							}),
						s.session2
					);

					// s is no more valid because s.session1 and s.session2 have been moved therefore dropped

					MeshedChannels {
						session1: channel_3_1,
						session2: channel_3_2,
						stack: stack_3,
						name: name_3,
					}
				} *@ \label{line:choice:end} @*
			\end{rustlisting}}
	\end{minipage}
	\begin{lstlisting}[label=lst:MPSTMeshedChannelsPrimitives, captionpos=b, caption=MPST Rust communication primitives]
\end{lstlisting}
	\caption{MPST Rust communication primitives}
	% \Description[MPST Rust communication primitives]{MPST Rust communication primitives}
	
\end{figure}

The order of usage of the binary channels of a \CODE{MeshedChannels} object is stored inside the \CODE{stack} field.
For instance, the behaviour that \role{A} has to communicate first with \role{B}, then with a \role{C}, and then the
session ends can be specified using a stack of type \CODE{RoleB<RoleC<RoleEnd>>}.
Note that all stack types, such as \CODE{RoleB}, \CODE{RoleC}, are generated.

\paragraph{\bf \MPST communication primitives as wrappers of binary channels.}
As explained in \textbf{\S~\ref{sec:overview}}, programming with~\mpstrust
relies on communication primitives, such as \CODE{send_mpst_a_to_b(s)},
that have the sender and receiver roles baked into their name.
To ensure that the binary channels are used as specified by the global protocol,
each communication function is parametric on a generic quadruple type
\CODE{<T, S1, S2, R>} where \CODE{T} is a payload type,
\CODE{S1} and \CODE{S2} are binary session types and
\CODE{R} is a type for a stack (\mpststack type) that imposes the order
in which the binary sessions inside a multiparty session must be
used.

\listing{lst:MPSTMeshedChannelsPrimitives} (lines~\ref{line:mpst:send} --~\ref{line:mpst:close}) shows
the implementation for \CODE{send_mpst_a_to_b(s)}. As clear from
the type parameters, the client of the function should supply a \mpststack
type \CODE{RoleB<R>}.
The binary session type \CODE{S1} should be encapsulated in a \CODE{Send<T, S1>}.
The body of the function sends the message of type \CODE{T}
on the binary channel stored in the first field, \CODE{session1} (corresponding to the binary
session with \role{B}), of the multiparty session \CODE{s}.
Since the communication is on a binary channel, we reuse the binary \CODE{send()} primitive from~\cite{kokkeRusty2019}.

External and internal choices are implemented as macros that require an argument of type \CODE{MeshedChannels}.
The implementation of the macro \CODE{offer_mpst_a_to_c!} is given in lines~\ref{line:offer:start} --~\ref{line:offer:end!}.
In essence, a choice is implemented as a broadcast from one role to the others.
In our usecase, the active role that makes the choice is \role{C}.
Hence, the macro \CODE{offer_mpst_a_to_c!} explicitly performs a receive (\CODE{recv_mpst_a_to_c(s)!}) on
the meshed channel \CODE{s}.
The received value is pattern matched and passed to any of the functions given as arguments to \CODE{offer_mpst_a_to_c!}.
Similarly, \CODE{choose_mpst_c_to_all!} in lines~\ref{line:choice:start} --~\ref{line:choice:end!} is a macro
that performs a select operation. The active \role{C} sends the selected label to all
roles in the protocol. In our particular example, \role{C} sends the selected label \CODE{l} to \role{A} and \role{B}.

\paragraph{\bf Discussions.}
Our implementation, although intuitive, does not resolve the inherent
conflict between Rust, which is \emph{affine}, and \emph{linear} session types. The implementation suffers from the same drawback as~\cite{kokkeRusty2019}. However, the \MPST
methodology is a step forward in terms of usability. Differently from
the Rust local types which can get convoluted, the syntax of global
protocols is user-friendly and readable. Developers can use the
global protocol as guidance, and hence avoid errors such as
prematurely ending of a session. Moreover, as observed in Kokke's
library~\cite{kokkeRusty2019}, most of the errors are caused by misuse
of methods and functions. Since we are code-generating the local
types, the chance of misspelling is significantly reduced.
Another viable option for our framework is to take the \emph{bottom-up} approach:
to check directly whether a set of manually-written Rust local types satisfy \emph{safety}/\emph{liveness} properties
by a model checker~\cite{scalasLess2019} or
the \emph{multiparty compatibility} (a property that guarantees
deadlock-freedom of communicating automata, which are equivalent to
local session types)~\cite{langeVerifying2019,denielouMultiparty2013}.


==> MPSTDef.tex <==
\section{Short Version}
\begin{restatable}[]{DEF}{defMPSTSyntax}\rm
\label{def:mpst-syntax-terms}
The \textbf{multiparty session $\pi$-calculus} syntax is defined as follows:%

\smallskip%
\centerline{$%
\begin{array}{r@{\hskip 2mm}c@{\hskip 2mm}l@{\hskip 2mm}l}
  %
  %
  \textstyle%
  \mpC, \mpD%
  &\coloncolonequals&%
  \mpFmt{x} \bnfsep \mpChanRole{\mpS}{\roleP}%
  & \mbox{\footnotesize(variable, channel with role $\roleP$)}
  \\[1mm]
  %
  %
  \mpP, \mpQ
  &\coloncolonequals&%
  \mpNil \;\bnfsep\; \mpP \mpPar \mpQ \;\bnfsep\; \mpRes{\mpS}{\mpP}%
  &
  \mbox{\footnotesize(inaction, composition, restriction)}
  \\
  &&
  \mpSel{\mpC}{\roleQ}{\mpLab}{\mpD}{\mpP}%
  &
  \mbox{\footnotesize(selection towards role $\roleQ$)}
  \\
  &&
  \mpBranch{\mpC}{\roleQ}{i \in I}{\mpLab[i]}{x_i}{\mpP[i]}%
  &
  \mbox{\footnotesize(branching from role $\roleQ$ with $I \neq \emptyset$)}
  \\
  &&
  \mpDefAbbrev{\mpDefD}{\mpP}%
  \bnfsep%
  \mpCall{\mpX}{\widetilde{\mpC}}
%  \bnfsep%
%  \mpErr%
  %
  &
  \mbox{\footnotesize(process definition, process call)}
  \\[1mm]
  %
  %
  \mpDefD%
  &\coloncolonequals&%
  \mpJustDef{\mpX}{\widetilde{x}}{P}
  &
  \mbox{\footnotesize(declaration of process variable $\mpX$)}
  \\[1mm]
\end{array}
$}
\end{restatable}



==> code-gen-macro.tex <==
% \begin{comment}
% \begin{figure}[t!]
%   \begin{minipage}[l]{0.4\textwidth}
%     \begin{rustlisting}[basicstyle=\scriptsize\ttfamily]
%       /// Binary session types for A and C
%       type RecvChoice<N> = *@\label{line:role:C:start}@*
%       Recv<ChoiceA<N>, End>;
%       type AtoCVideo<N> =
%       Recv<N, Send<N, RecvChoice<N>>
%       type AtoCClose = End; *@\label{line:role:C:end}@*

%       /// Binary session types for A and B
%       type AtoBVideo<N> = *@\label{line:role:B:start}@*
%       Send<N, Recv<N, End>>;
%       type AtoBClose = End; *@\label{line:role:B:end}@*

%       /// Declare usage order of channels
%       type StackAInit = RoleC<RoleC< *@\label{line:role:stacks:start1}@*
%       RoleC<RoleEnd>>>;
%       type StackAChoice = RoleC<RoleEnd>;

%       /// Declare the name of the role
%       type NameA = RoleA<RoleEnd> *@\label{line:role:stacks:name}@*
%     \end{rustlisting}
%   \end{minipage}
%   \begin{minipage}[l]{0.3\textwidth}
%     {\lstset{numbers=none}
%       \begin{SCRIBBLELISTING}[basicstyle=\scriptsize\ttfamily,numbers=none]
%         local protocol VideoPRec
%         at A(role B, role C){
%             choice at C {
%                 VideoRequest(
%                 string) from C;
%                 VideoRequest(
%                 string) to B;
%                 SendVideo(Video) from B;
%                 SendVideo(Video) to C;
%                 do VideoPRec(B, C);
%               } or {

%                 Close() from C;
%                 Close() to B, C;
%               }}
%       \end{SCRIBBLELISTING}}
%   \end{minipage}
%   \begin{minipage}[r]{0.35\textwidth}
%     \begin{tikzpicture}[
%         role/.style={circle,text width=1.5em,text centered,draw,inner sep=0,font=\small},
%         arrow/.style={>=latex,thick,draw},
%         label/.style={inner sep=0,font=\sf\small},
%         transform shape,
%         scale = 0.8
%       ]
%       \node (a1) [role]{$s_1$};
%       \node (a2) [role,right=1.3 of a1] {$s_2$};
%       \node (a3) [role,left=1.3 of a2] {$s_1$}
%       edge [arrow,->, bend left] node [midway,yshift=5pt,label] {$m1\ptp{A}\ptp{B}$} (a2);
%       \node (a4) [role,right=1.3 of a2] {$s_3$}
%       edge [arrow,->, bend left] node [midway,yshift=5pt,label] {$m4!\ptp{A}\ptp{B}$} (a1)
%       edge [arrow,->, bend left] node [midway,yshift=5pt,label] {$m3!\ptp{A}\ptp{B}$} (a2);
%       \node (a5) [role,right=1.3 of a1] {$s_2$}
%       edge [arrow,->, bend left] node [midway,yshift=5pt,label] {$m2!\ptp{A}\ptp{B}$} (a4);
%       %draw[arrow,->, bend left] edge (a1) -- (a2);
%       %    edge [arrow,<-, bend left] node [midway,yshift=5pt,label] {$msg!\ptp{A}\ptp{B}$} (a2);
%       %   	edge [arrow, bend left] (a1) {msg};
%     \end{tikzpicture}
%     \begin{tikzpicture}[
%         role/.style={circle,text width=1.5em,text centered,draw,inner sep=0,font=\small},
%         arrow/.style={>=latex,thick,draw},
%         label/.style={inner sep=0,font=\sf\small},
%         transform shape,
%         scale = 0.8
%       ]
%       \node (a1) [role]{$s_1$};
%       \node (a2) [role,right=1.3 of a1] {$s_2$};
%       \node (a3) [role,left=1.3 of a2] {$s_1$}
%       edge [arrow,->, bend left] node [midway,yshift=5pt,label] {$m1\ptp{A}\ptp{B}$} (a2);
%       \node (a4) [role,right=1.3 of a2] {$s_3$}
%       edge [arrow,->, bend left] node [midway,yshift=5pt,label] {$m4!\ptp{A}\ptp{B}$} (a1)
%       edge [arrow,->, bend left] node [midway,yshift=5pt,label] {$m3!\ptp{A}\ptp{B}$} (a2);
%       \node (a5) [role,right=1.3 of a1] {$s_2$}
%       edge [arrow,->, bend left] node [midway,yshift=5pt,label] {$m2!\ptp{A}\ptp{B}$} (a4);
%       %draw[arrow,->, bend left] edge (a1) -- (a2);
%       %    edge [arrow,<-, bend left] node [midway,yshift=5pt,label] {$msg!\ptp{A}\ptp{B}$} (a2);
%       %   	edge [arrow, bend left] (a1) {msg};
%     \end{tikzpicture}
%     \begin{tikzpicture}[
%         role/.style={circle,text width=1.5em,text centered,draw,inner sep=0,font=\small},
%         arrow/.style={>=latex,thick,draw},
%         label/.style={inner sep=0,font=\sf\small},
%         transform shape,
%         scale = 0.8
%       ]
%       \node (a1) [role]{$s_1$};
%       \node (a2) [role,right=1.3 of a1] {$s_2$};
%       \node (a3) [role,left=1.3 of a2] {$s_1$}
%       edge [arrow,->, bend left] node [midway,yshift=5pt,label] {$m1\ptp{A}\ptp{B}$} (a2);
%       \node (a4) [role,right=1.3 of a2] {$s_3$}
%       edge [arrow,->, bend left] node [midway,yshift=5pt,label] {$m4!\ptp{A}\ptp{B}$} (a1)
%       edge [arrow,->, bend left] node [midway,yshift=5pt,label] {$m3!\ptp{A}\ptp{B}$} (a2);
%       \node (a5) [role,right=1.3 of a1] {$s_2$}
%       edge [arrow,->, bend left] node [midway,yshift=5pt,label] {$m2!\ptp{A}\ptp{B}$} (a4);
%       %draw[arrow,->, bend left] edge (a1) -- (a2);
%       %    edge [arrow,<-, bend left] node [midway,yshift=5pt,label] {$msg!\ptp{A}\ptp{B}$} (a2);
%       %   	edge [arrow, bend left] (a1) {msg};
%     \end{tikzpicture}
%   \end{minipage}
%   \begin{lstlisting}[label=lst:UsecaseDeclarationTypes, captionpos=b]
% \end{lstlisting}
%   \caption{Local Rust types for role A}
% \end{figure}
%\paragraph{\bf Handling cancellation}
%\paragraph{\bf The gap between theory and implementation} What is the argument that the implementation is faithful to the theory

%\paragraph{\bf Extension}
% Our implementation, although intuitive, does not resolve the inherent
%conflict between Rust, which is \emph{affine}, and session types, which are
%\emph{linear}. The implementation suffers from the same drawback as~\cite{kokkeRusty2019}.
% However, the \MPST
%methodology is a step forward in terms of usability.
% Differently than
%the Rust local types which can get convoluted, the syntax of global
%protocols is user-friendly and readable.
% Developers can use the
%global protocol as guidance, and hence avoid errors such as
%prematurely ending of a session.
% Moreover, as observed in Kokke's
%library~\cite{kokkeRusty2019}, most of the errors are caused by misuse
%of methods and functions.
% Since we are code-generating the local
%types, the chance of misspelling is significantly reduced.
% Another viable option for our framework is to take the \emph{bottom-up} approach:
% to check directly whether a set of manually-written Rust local types satisfy
%\emph{safety}/\emph{liveness} properties by a model checker~\cite{scalasless2019} or
%the \emph{multiparty compatibility} (a property which guarantees
%deadlock-freedom of communicating automata, which are equivalent to
%local session types)~\cite{langeverifying2019,denieloumultiparty2013}.

% \begin{figure}[b!]
%   \begin{minipage}{0.5\textwidth}
%     {\small
%       \begin{cdescription}[leftmargin=*]
%         \item[Output] $\delta(s) = \SET{\alpha^!_i}_{1..n}, n>0$: the STP generates
%         %has ${\geq}1$ $!$-actions:

%         \quad\fCODE{type }$\encc{s}$\fCODE{ = }$m_1$ $\dots$ $m_n$

%         \noindent
%         ~~where for each $\alpha_i = r_i ! \lbl_i (T_i); $,

%         \quad $m_i =${ member Send}$: r_i \rightarrow \lbl_i \rightarrow \mathtt{T_i} \rightarrow \encc{\delta(s, \alpha_i)}$

%         \medskip

%         \item[Single-input] $\delta(s) = \SET{r ? l (T); \mathtt{\sigma;}\ $}: the STP generates
%           %$s$ has one $?$-action.

%           \quad{type }$\encc{s} =$ {member Receive:}$r \rightarrow \lbl \rightarrow \mathtt{T} \rightarrow \encc{\delta(s, \alpha)}$

%         \medskip
%       \end{cdescription}}
%   \end{minipage}
%   \begin{minipage}{0.45\textwidth}
%     {\small
%       \begin{cdescription}[leftmargin=*]
%         \item[Output] $\delta(s) = \SET{\alpha^!_i}_{1..n}, n>0$: the STP generates
%         %has ${\geq}1$ $!$-actions:

%         \quad{type }$\encc{s}${ = }$m_1$ $\dots$ $m_n$

%         \noindent
%         ~~where for each $\alpha_i = r_i ! \lbl_i (T_i);$,

%         \quad $m_i =${ member Send}$: r_i \rightarrow \lbl_i \rightarrow \mathtt{T_i} \rightarrow \encc{\delta(s, \alpha_i)}$

%         \medskip

%         \item[Single-input] $\delta(s) = \SET{r ? l (T); \mathtt{\sigma;}\ $}: the STP generates
%           %$s$ has one $?$-action.

%           \quad{type }$\encc{s} =$ {member Receive:}$r \rightarrow \lbl \rightarrow \mathtt{T} \rightarrow \encc{\delta(s, \alpha)}$

%         \medskip
%       \end{cdescription}}
%   \end{minipage}
%   \caption{Pseudocode for code generation}
% \end{figure}

% \subsection{Code Generation: From Scribble Protocols to Rust Types}
% \textbf{Global Protocols in Scribble.}~\Cref{fig:CreateMeshedChannels} explains the code generation utility that translates scribble protocol types to Rust types. We show the generation from CFSM, for convenience. The pseudo code of the generation is given in Fig. X. Which is the insights that allows us to handle cancellation.
% The return type of all functions is \CODE{Result<Box...>}
% Everything below is simply a filler...
% We use macros to bake the names into the functions ? a library for code generating primitives for multiparty session types. The tool takes a mapping m from from role names to indexes.
% A simple representation of the mapping is available on the rights, and it generates the power set of all primitives.
% Note that not all of these primitives will be needed, and indeed, if the code is generated from Scribble, the generated code will be reduces.
% We use macros to bake the names into the functions ? a library for code generating primitives for multiparty session types. The tool takes a mapping m from from role names to indexes.
% A simple representation of the mapping is available on the rights, and it generates the power set of all primitives.

% \textbf{Code Generation.} Note that not all of these primitives will be needed, and indeed, if the code is generated from Scribble, the generated code will be reduces.
% We use macros to bake the names into the functions ? a library for code generating primitives for multiparty session types. The tool takes a mapping m from from role names to indexes.
% A simple representation of the mapping is available on the rights, and it generates the power set of all primitives.
% Note that not all of these primitives will be needed, and indeed, if the code is generated from Scribble, the generated code will be reduces.
% Here we show several example of how cancellation can be handled.
% An example of a code that will be generated from the protocols \CODE{msg() from A to B; msg() from B to C;} is ...the types below...Fig. X shows the protocol from our running example in Scribble, and as a CFSM.~\Cref{fig:CreateMeshedChannels} demonstrated the types that are generated.
% We should show the cfsm and the generated types.
% \textbf{Example.} Note that not all of these primitives will be needed, and indeed, if the code is generated from Scribble, the generated code will be reduces.
% We use macros to bake the names into the functions ? a library for code generating primitives for multiparty session types. The tool takes a mapping m from from role names to indexes.
% A simple representation of the mapping is available on the rights, and it generates the power set of all primitives.
% Note that not all of these primitives will be needed, and indeed, if the code is generated from Scribble, the generated code will be reduces.
% Here we show several example of how cancellation can be handled.
% An example of a code that will be generated from the protocols \CODE{msg() from A to B; msg() from B to C;} is ...the types below...Fig. X shows the protocol from our running example in Scribble, and as a CFSM. Listing X demonstrated the types that are generated.
% We should show the cfsm and the generated types.

% \newcommand{\RHCHECK}[1]{#1}
% \newcommand{\LSENDrl}[1]{#1}
% \newcommand{\LRECVrl}[1]{#1}

% \begin{figure*}[t!]
%   \newcommand{\CHSKIP}{10mm}
%   \newcommand{\sendarrow}{\draw[->, draw=blue]}
%   \newcommand{\recvarrow}{\draw[->, draw=red, dashed]}

%   %\hspace{-3pt}
%   \begin{tabular}{p{0.46\textwidth} ll}
%     \adjustbox{valign=t}{%
%       \begin{tikzpicture}%[every edge/.append style = {->,x=0.8cm, y=2cm, bend angle=35, raw=blue, dotted, thick}]
%         [
%           >=stealth',
%           STATE/.style={draw,circle,inner sep=0pt,minimum width=4.5mm}
%         ]
%         \node[STATE] (s1) {\footnotesize$1$};
%         %
%         \node[STATE, right=13mm of s1] (s2) {\footnotesize$2$};
%         \node[STATE,right=15mm of s2] (s3) {\footnotesize$3$};
%         \node[STATE,right=\CHSKIP of s3] (s4) {\footnotesize$4$};
%         \node[STATE,right=\CHSKIP of s4] (s5) {\footnotesize$5$};
%         \node[STATE,below=\CHSKIP of s5] (s6) {\footnotesize$6$};
%         %
%         \node[STATE,below=3mm of s4] (s7) {\footnotesize$7$};
%         \node[STATE,below=10mm of s3] (s8) {\footnotesize$8$};
%         %
%         \node[STATE,below=5mm of s6] (s9) {\footnotesize$9$};
%         \node[STATE,below=20mm of s2] (s10) {\footnotesize$10$};
%         %
%         \node[STATE,below=10mm of s1] (s11) {\footnotesize$11$};
%         \node[STATE, below=5mm of s11] (s12) {\footnotesize$12$};
%         %
%         %
%         \sendarrow (s1) -- node[above,pos=0.8]{\footnotesize$\alpha_1$} (s2);
%         \sendarrow (s2) -- node[above,pos=0.7]{\footnotesize$\alpha_2$} (s3);
%         \recvarrow (s3) -- node[above]{\footnotesize$\alpha_3$} (s4);
%         \sendarrow (s4) -- node[above]{\footnotesize$\alpha_4$} (s5);
%         \recvarrow (s5) -- node[above,pos=0.7,xshift=7pt]{\footnotesize$\alpha_5$} (s6);
%         %
%         \sendarrow (s6) to[bend right=20] node[above] {\footnotesize$\alpha_6$} (s7);
%         \sendarrow (s7) to[bend left=20] node[above] {\footnotesize$\alpha_7$} (s2);
%         %
%         \sendarrow (s6) to[bend left=0] node[above] {\footnotesize$\alpha_8$} (s8);
%         \sendarrow (s8) to[bend left=20] node[above] {\footnotesize$\alpha_9$} (s2);
%         %
%         \sendarrow (s6) to[bend left=0] node[above,pos=0.9, xshift=7pt] {\footnotesize$\alpha_{10}$} (s9);
%         \recvarrow (s9) -- node[above]{\footnotesize$\alpha_{11}$} (s10);
%         \sendarrow (s10) to[bend right=15] node[above,pos=0.2, xshift=8pt] {\footnotesize$\alpha_{12}$} (s2);
%         \sendarrow(s10) to[bend left=15] node[below,pos=0.4, xshift=-8pt] {\footnotesize$\alpha_{13}$} (s2);
%         %
%         \sendarrow (s2) -- node[above,pos=0.7,xshift=-2pt]{\footnotesize$\alpha_{14}$} (s11);
%         \sendarrow (s11) -- node[above,pos=0.7,xshift=-7pt]{\footnotesize$\alpha_{15}$} (s12);
%       \end{tikzpicture}
%     }
%      &
%     %\hspace{-17pt}
%     \adjustbox{valign=t}{%
%       \footnotesize
%       $\begin{array}{l}
%           \alpha_1=\LSENDrl{\MCODE{R}}{\MCODE{Plane(\RHCHECK{p},}\MCODE{\RHCHECK{p},}\MCODE{\RHCHECK{p},}\MCODE{\RHCHECK{p})}} \\
%           \alpha_2=\LSENDrl{\MCODE{R}}{\MCODE{IsAbove(v1:\RHCHECK{p})}}                                                        \\
%           \alpha_3=\LRECVrl{\MCODE{R}}{\MCODE{Res(b1:b)}}                                                                      \\
%           \alpha_4=\LSENDrl{\MCODE{R}}{\MCODE{IsAbove(v2:\RHCHECK{p})}}                                                        \\
%           \alpha_5=\LRECVrl{\MCODE{R}}{\MCODE{Res(b2:b)}}                                                                      \\
%           \alpha_6=\LSENDrl{\MCODE{C}}{\MCODE{BothIn(}x_1\MCODE{)}};                                                           \\
%           \alpha_7=\LSENDrl{\MCODE{R}}{\MCODE{BothIn()}}                                                                       \\
%         \end{array}$
%     }
%      &
%     \adjustbox{valign=t}{%
%       \footnotesize
%       $\begin{array}{l}
%           \alpha_8=\LSENDrl{\MCODE{C}}{\MCODE{BothOut()}};              \\
%           \alpha_9=\LSENDrl{\MCODE{R}}{\MCODE{BothOut()}}               \\
%           \alpha_{10}=\LSENDrl{\MCODE{R}}{\text{$\MCODE{Intrsct()}$}};  \\
%           \alpha_{11}=\LRECVrl{\MCODE{R}}{\MCODE{Res(i:P)}}             \\
%           \alpha_{12}=\LSENDrl{\MCODE{C}}{\MCODE{SecOut(}x_2\MCODE{)}}; \\
%           \alpha_{13}=\LSENDrl{\MCODE{C}}{\MCODE{SecIn(}x_3\MCODE{,} x_4\MCODE{)}};%\\ \hspace{7mm}
%           \\
%           \alpha_{14}=\LSENDrl{\MCODE{R}}{\MCODE{Close()}}              \\
%           \alpha_{15}=\LSENDrl{\MCODE{C}}{\MCODE{Close()}}              \\
%         \end{array}$}
%     %&
%     %\adjustbox{valign=t}{%
%     %\footnotesize
%     %$\begin{array}{l}
%     %\alpha_{10}=\LSENDrl{\MCODE{R}}{\MCODE{IntrSct()}}; \MCODE{b1} \!\oplus\! \MCODE{b2} \\
%     %\alpha_{14}=\LSENDrl{\MCODE{R}}{\MCODE{Close}} \\
%     %\alpha_{15}=\LSENDrl{\MCODE{C}}{\MCODE{Close}} \\
%     %\end{array}$}
%   \end{tabular}
%   %
%   \caption{CFSM representation of role \fCODE{A} from protocol \fCODE{Stream} in~\Cref{fig:scr:SH} ($\color{blue}{\rightarrow}$ denotes
%     an output, $\color{red}{\dashrightarrow}$ is an input)}
%   %
%   \label{fig:cfsm}
%   %
%   \caption{CFSM for the running example}
% \end{figure*}
% \end{comment}

\subsection{Code generation:~\mpstrust for an arbitrary number of roles}
Currently, we have only demonstrated a communication API for three hard-coded roles, but our code generation facilities
provide utility functions for generating API for an arbitrary number of roles, parametric on the role names.
In essence, each generated function is a
generalisation of the functions presented in~\Cref{fig:CreateMeshedChannels}.
We will show only the most important of the code-generation functions -- the one that generates a new \AMPST structure.
All utility functions are implemented as Rust macros.
Rust supports two types of macros -- regular and procedural, we utilise both.
The former are expanded into a syntactic form during compilation,
before any static checking, while the latter is a function over the Rust AST and creates syntax extensions.
% They allow to run code at compile time that operates over Rust
%syntax, both consuming and producing Rust syntax.
%\ie they are functions from an Abstract Syntax Tree to an Abstract Syntax Tree.
% Hence, we create macros that generate the function for send, recv, choose and offer but are parametric on role name.
% To create a new function adapted to our new role, we need to provide the name of the new function,
% the role that will be consumed and the name of the role that will apply this function

\input{fig-matrix}

~\Cref{fig:CreateMeshedChannels} (left) shows the macro that generates \MPST structure with an arbitrary number of
roles,~\Cref{fig:CreateMeshedChannels} (right) shows its usage for creating \MPST structure with four participants,
along with the generated structure.
The macro inputs for the regular macro (line~\ref{line:meshedchannels:multiple:regular:call})
are the name of the structure and the number of roles, and are passed to the procedural macro.
\CODE{mpst_seq::create_meshedchannels} calls a method
that creates the code with \CODE{quote!}, using the arguments provided by the user.
After retrieving the arguments,
the macro creates the different groups of \CODE{ident},
such as \emph{sessions} (line~\ref{line:meshedchannels:multiple:procedural:meshedchannels:vec:sessions}).
Those \CODE{Vec} contain the blocks of code that are repeated,
such as \CODE{S1 , S2 , S3 ,}, \dots
for \CODE{sessions}.
The \CODE{...} at line~\ref{line:meshedchannels:multiple:procedural:meshedchannels:rest:vec} materialises the other \CODE{Vec} that are created.
Those groups are concatenated along with complementary code between lines~\ref{line:meshedchannels:multiple:procedural:meshedchannels:quote:start}
and~\ref{line:meshedchannels:multiple:procedural:meshedchannels:quote:end}.
The rest of the code, materialised with \CODE{...}
at line~\ref{line:meshedchannels:multiple:procedural:meshedchannels:rest:quote},
contain the methods for the new structure.
The line~\ref{line:meshedchannels:multiple:regular:call} displays the usage of the regular macro for developers,
and the code created for 4 participants is show between lines~\ref{line:meshedchannels:multiple:structure:created:start}
and~\ref{line:meshedchannels:multiple:structure:created:end}.

% \CODE{seq!} is a procedural macro that iterates over a block of code.
% In particular, the code inside \textbf{\#(...)} iterates over \CODE{N}.
% For instance, at line~\ref{line:meshedchannels:multiple:loop}, the code
% \CODE{S#N:0: mpstthree::binary::Session} will be repeated 4 times if \CODE{nsessions} equals 4.
% Furthermore, in such block of code, every time there is the symbol \textbf{\#} immediately followed by the name of the index,
% then, this specific code will be replaced by the loop index.
% For instance, the line~\ref{line:meshedchannels:multiple:generatedSessionTypes}, alongside the symbols \textbf{\#()} which encapsulate
% it, will be replaced by the ones given in~\Cref{fig:CreateMeshedChannels}.
% Besides those two loops, the rest of the visible code remains untouched by the procedural macro.
% This method allows for the creation of multiple binary meshed channels, one \emph{stack} and one \emph{name} fields.

% \newpage

% The tool takes a mapping m from from role names to indexes.
\begin{wrapfigure}{r}{0.2\textwidth}
	\begin{tabular}{l " l | l | l | l }
		  & a  & b  & c  & d \\
		\thickhline
		a &    & 1  & 2  & 3 \\
		\hline
		b & -1 &    & 4  & 5 \\
		\hline
		c & -2 & -4 &    & 6 \\
		\hline
		d & -3 & -5 & -6 &
	\end{tabular}
	% \Description[Distribution of the channels for \emph{branching} for 4 participants]{
	% 	Distribution of the channels for \CODE{branching} for 4 participants}
	\caption{Distribution of the channels for \CODE{branching} for 4 participants}
	\label{fig:choose:multiple:distribution}
	
\end{wrapfigure}

The most intricate part when implementing multiparty channel is the mapping between binary
channels and their name in their index in the \MPST structure.
When the session starts, all the newly created binary channels should be correctly distributed among all roles.
We will rely on the kind of structure displayed in~\Cref{fig:choose:multiple:distribution}.
The figure demonstrates the distribution for a protocol involving 4 roles.
The headers, column and row, contain the different roles, and the rest details the index of the channels between two participants.
This is a skew-symmetric matrix, where each number on the top right has an opposite in the bottom left.
A negative number means that the role on the corresponding row will receive the dual
of the binary session type of the role on the corresponding column.

% Consider the case of 5 participants, (A, B, C, D and E), which generates the different endpoints for B and D, considering that are given in~\Cref{lst:Endpoints5ParticipantsBandD}.
% To generate the new structure \CODE{MeshedChannels} given in~\Cref{lst:Endpoints5ParticipantsBandD}, we implemented the macro
%\CODE{create_meshedchannels!}.
% Its inputs are the name of the new structure and the number of participants, and a part of the code can be seen in
%~\Cref{fig:CreateMeshedChannels}.
% This code is divided in 2 nested parts:
%
%\begin{itemize}
%	\item The \CODE{macro_rules!} named \CODE{create_meshedchannels!}, which is the one called by the user.
%	      Its inputs are, respectively, the name of the new \CODE{MeshedChannels} and the number of participants
%	\item \CODE{seq!}, a procedural macro from the complementary library \CODE{mpst_seq!}
%	      that we created, which requires three arguments: the name of an index (\CODE{N} here) and two bounds (1 and \CODE{nsessions}).
%\end{itemize}

==> oauth.tex <==
\section{OAuth2 protocol}
\label{sec:oauth}

In this section, we introduce the implementation of the OAuth2 protocol.
First, we detail the official protocol according to the official website \footnote{\url{https://oauth.net/2/}},
then we explain how it was implemented in Scribble then in~\mpstrust.

\subsection{The official protocol}
\label{subsec:oauth2:OfficialProtocol}

\begin{figure}[t!]
	\includegraphics[scale=0.8]{pdf/oauth2.pdf}
	\caption{OAuth2 protocol}
	% \Description[Description of the OAuth2 protocol]{Description of the OAuth2 protocol}
	\label{fig:oauth2}
\end{figure}

The OAuth protocol requires 4 entities and works in 6 main steps: a \emph{Client} requests an \emph{Authorization Approval} to a
\emph{Resource Owner}, transmits it to an \emph{Authorization server} to get an \emph{Access Token}.
This \emph{Access Token} allows the \emph{Client} to request \emph{Protected Resources}, such as pictures, videos or messages.
The scheme of this protocol can be seen in~\Cref{fig:oauth2}.
Usually, due to security reasons, the communications with the \emph{Resource Owner} need to be \emph{human certified}: the
request needs to be completed by a human through a \emph{captcha} or any steps that can be completed \emph{only by humans}.
Because of this restriction, we will omit those interactions in the implementation of the protocol.

\subsection{Implementation}

\lstinputlisting[%	
	language=Scribble,style=ScribbleWithLN,basicstyle=\scriptsize\ttfamily,%
	firstline=1,lastline=35,%
	float,%
	label=lst:oauth-protocol,%
	caption=Main body of the OAuth protocol in Scribble,%
]{protocols/OAuth.scr}

Following the consideration above, you can find the Scribble protocol in~\Cref{lst:oauth-protocol}.
It closely follows the official protocol, with 3 roles (\role{Auth}, \role{Client} and \role{Server}),
and the loop for either requesting protected resources or closing the connection.

We used the Imgur api \url{https://api.imgur.com/} for the test, which implements the OAuth2 protocol.
After retrieving the \emph{Authorization Approval} from the Imgur server, we modified the \CODE{send()}
and \CODE{recv()} functions to handle https communications.
We used the \emph{hyper} crate\footnote{\url{https://docs.rs/hyper/}} for basic http communications,
alongside the \emph{hyper-tls} crate\footnote{\url{https://docs.rs/hyper-tls/}} for the secured communications.
We directly went for macros to create functions that accept the
roles that we wanted, no matter how many there are.
We created the macros \CODE{create_send_http_session!} and \CODE{create_recv_http_session!}
which encapsulate, resp., a way to create send and receive \emph{REQUEST}.
The generated functions will look like the ones in~\Cref{lst:SendRecvHttp}.

\begin{minipage}[l]{0.5\textwidth}
	\begin{rustlisting}[label=lst:send:http]
		fn send_http(payload: T, s: MeshedChannels<...>, req: hyper::Request) -> (MeshedChannels<...>, hyper::client::ResponseFuture) {
				let https = hyper_tls::HttpsConnector::new();
				let client = hyper::Client::builder().build::<_, hyper::Body>(https);
				let respfuture = client.request(req);

				...

				(new_meshedchannels, respfuture)
			}
	\end{rustlisting}
\end{minipage}
\begin{minipage}[r]{0.5\textwidth}
	\begin{rustlisting}[label=lst:recv:http]
		fn recv_http(payload: T, s: MeshedChannels<...>, respfuture: hyper::client::ResponseFuture) -> Result<(MeshedChannels<...>, hyper::Response), Box<dyn std::error::Error>> {
				let rt = tokio::runtime::Runtime::new()?;
				let resp = rt.block_on(async move { respfuture.await })?; *@\label{line:http:recv:wait}@*

				...

				Ok((new_meshedchannels, resp))
			}
	\end{rustlisting}
\end{minipage}
\begin{lstlisting}[label=lst:SendRecvHttp, captionpos=b, caption=Rust implementation of the
	macros \CODE{create\_send\_http_session!} and \CODE{create\_recv\_http_session!}]
\end{lstlisting}

As you may notice, there is the usage of the \CODE{async} Rust feature, which is the Rust way
to implement a \emph{concurrent programming model}.
We do not extensively use it in our library because it conflicts with the usage of the threads, that
is why we immediately block on it and wait for the answer with the line~\ref{line:http:recv:wait}.
Currently, the developers have to provide a \CODE{hyper::Request} to the \CODE{send()}
functions, which requires basic knowledge about the \CODE{hyper} library.
In~\Cref{lst:http:request}, we detail the creation of a \emph{Request}.
Such element contains a method (line~\ref{line:http:request:method}), an uri (line~\ref{line:http:request:uri}), headers
(lines~\ref{line:http:request:header:start} to~\ref{line:http:request:header:end}) and a
body (line~\ref{line:http:request:body}).
In our case, we use the \emph{GET} method to request resources.
The fields provided with \emph{ids} are stored in a \emph{.env} file which is only stored locally for security purpose.
The uri depends on the resources we want to retrieve: in our case, it will look like \emph{https://api.imgur.com/3/XXX}.
Here, the body is empty, as seen with \CODE{Body::default()}, but for a \emph{POST}, it may not be empty.

\begin{minipage}[l]{\textwidth}
	\begin{rustlisting}[label=lst:send:http]
		let mut ids: HashMap<&str, &str> = HashMap::with_hasher(hasher); // Create and fill a hasmap with the required token for the OAuth protocol

		let req = Request::builder()
			.method(Method::GET) *@\label{line:http:request:method}@*
			.uri(ids["CREDITS_URL"]) *@\label{line:http:request:uri}@*
			.header("content-type", ids["CONTENT_TYPE"]) *@\label{line:http:request:header:start}@*
			.header(
				"Authorization",
				format!("{} {}", ids["TOKEN_TYPE"], ids["ACCESS_TOKEN"]),
			)
			.header("User-Agent", ids["USER_AGENT"])
			.header("Accept", ids["ACCEPT"])
			.header("Connection", ids["CONNECTION"]) *@\label{line:http:request:header:end}@*
			.body(Body::default())?; *@\label{line:http:request:body}@*
	\end{rustlisting}
\end{minipage}
\begin{lstlisting}[label=lst:http:request, captionpos=b, caption=Creating a \emph{hyper Request}]
\end{lstlisting}

The number of available requests to this api with our own token can be retrieved by sending a GET request
to the uri \url{https://api.imgur.com/3/credits} and in our case, we receive this response,
in~\Cref{lst:response:json}.
\begin{lstlisting}[label=lst:response:json, escapeinside={*@}{@*}, captionpos=b, caption=JSON reponse]
{
	"data": { *@\label{line:lst:response:json:data}@*
		"UserLimit": 2000,
		"UserRemaining": 1998,
		"UserReset": 1617368318,
		"ClientLimit": 12500,
		"ClientRemaining": 12498
	},
	"success": true, *@\label{line:lst:response:json:success}@*
	"status": 200 *@\label{line:lst:response:json:status}@*
}
\end{lstlisting}

This is a \emph{JSON} containing 3 main fields: \emph{data}, \emph{success} and \emph{status}.
The two last ones (lines~\ref{line:lst:response:json:success} and~\ref{line:lst:response:json:status}) specify
how the whole communication went.
Here, according to those files, the whole communication went successful and we received the requested resources.
The field \emph{data} (line~\ref{line:lst:response:json:data}) contains the requested resources: the credits left for using the api.

As seen in this section, our tool can be used for testing protocols in other environments such as \emph{http} and \emph{https}.
We also added the \emph{TCP} support, with similar modifications of the \CODE{send()} and \CODE{recv()} functions.

==> old_AMPST.tex <==
\section{Affine multiparty session processes for Rust programming}
\label{sec:MPST}
\subsection{Affine multiparty session processes}
\label{subsec:processes}
Our calculus (\AMPST) is an extension of a full multiparty session
$\pi$-calculus~\cite{scalasLess2019} which includes session delegation
(channel passing) and session recursion.
We shade additions to~\cite{scalasLess2019} in\colorbox{ColourShade}{this colour}.

\begin{restatable}[]{DEF}{defMPSTSyntax}\rm
  \label{def:mpst-syntax-terms}
  The \textbf{affine multiparty session $\pi$-calculus} (\AMPST) is defined as follows:%

  \smallskip%
  \centerline{$%
      \begin{array}{r@{\hskip 2mm}c@{\hskip 2mm}l@{\hskip 2mm}l}
        %
        %
        \textstyle%
        \mpC, \mpD%
         & \coloncolonequals                                                       & %
        \mpFmt{x} \bnfsep \mpChanRole{\mpS}{\roleP} \bnfsep \chanraise%
        \quad\quad
        \colorbox{ColourShade}{$\mpDagger$}%
        \coloncolonequals
        \colorbox{ColourShade}{$\emptyset \bnfsep \mpQuestion$}
         & \mbox{\footnotesize(variable, channel with role $\roleP$, error, flag)}
        \\[1mm]
        %
        %
        \mpP, \mpQ
         & \coloncolonequals                                                       & %
        \mpNil \;\bnfsep\; \mpP \mpPar \mpQ \;\bnfsep\; \mpRes{\mpS}{\mpP}%
         &
        \mbox{\footnotesize(inaction, composition, restriction)}
        \\
         &
         &
        \colorbox{ColourShade}{$\mpQuestionSel{\mpC}{\roleQ}{\mpLab}{\mpD}{\mpP}$}%
        \bnfsep
        \colorbox{ColourShade}{$\mpQuestionBranch{\mpC}{\roleQ}{i \in I}{\mpLab[i]}{x_i}{\mpP[i]}$}%
         &
        \mbox{\footnotesize(affine selection, branching $I \neq \emptyset$)}
        \\
         &                                                                         &
        \;\;\;
        \mpSel{\mpC}{\roleQ}{\mpLab}{\mpD}{\mpP}%
        \;\bnfsep\;\;\;\;
        %  &
        %  \mbox{\footnotesize(selection towards role $\roleQ$)}
        %  \\
        %  &&
        \mpBranch{\mpC}{\roleQ}{i \in I}{\mpLab[i]}{x_i}{\mpP[i]}%
         &
        \mbox{\footnotesize(selection, branching $I \neq \emptyset$)}
        \\
         &                                                                         &
        \;\;\;
        \mpDefAbbrev{\mpDefD}{\mpP}%
        \bnfsep%
        \;\;\;
        \mpCall{\mpX}{\widetilde{\mpC}}
         & \mbox{\footnotesize(process definition, process call)}
        \\
         &                                                                         &
        \colorbox{ColourShade}{$\trycatch{P}{Q}$}%
        \bnfsep%
        \colorbox{ColourShade}{$\mpCancel{\mpC}{\mpP}$}
        \bnfsep%
        \colorbox{ColourShade}{$\kills{\mpS}$}
        % \bnfsep%
        % \mpErr%
        %
         &
        \mbox{\footnotesize(catch, cancel, kill)}
        \\[1mm]
        %
        %
        \mpDefD%
         & \coloncolonequals                                                       & %
        \mpJustDef{\mpX}{\widetilde{x}}{P}
         &
        \mbox{\footnotesize(declaration of process variable $\mpX$)}
        \\[1mm]
      \end{array}
    $}
\end{restatable}
\noindent
A set $\PSet$ denotes \textbf{participants}: $\PSet =\{\roleP, \roleQ, \roleR, \dots\}$,
and $\ASigma$ is a set of alphabets.
A \textbf{channel $\mpC$} can be either a variable;
a \textbf{channel with role $\mpChanRole{\mpS}{\roleP}$}, %
\ie a multiparty communication endpoint %
whose user plays role $\roleP$ in the session $\mpS$; or
a constant channel \textbf{err} corresponds to the situations in
\Cref{fig:implementation:role:a,fig:implementation:role:c} -- timeout on a channel or
incorrect implementations such as expression errors
that explicitly triggers the exception.
$\widetilde{\mpC}$ denotes a vector $c_1c_2\dots c_n$ ($n\leq 0$)
and similarly for $\widetilde{x}$ and $\widetilde{s}$.

Next two processes with $\mpQuestion$ model the option \texttt{?} in
Rust.
Process $\mpQuestionSel{\mpC}{\roleQ}{\mpLab}{\mpD}{\mpP}$ performs an %
\textbf{affine selection (internal choice)} %
towards role $\roleQ$, %
using the channel $\mpC$: %
if the \emph{message label} $\mpLab$ with the \emph{payload} channel
$\mpD$ is successfully sent, %
and the execution continues as $\mpP$; otherwise (if the receiver
has failed or timeout), it triggers the exception.
The %
\textbf{affine branching (external choice)}
$\mpQuestionBranch{\mpC}{\roleQ}{i \in I}{\mpLab[i]}{x_i}{\mpP[i]}$ %
uses channels $\mpC$ to wait for a message %
from role $\roleQ$: %
if a message label $\mpLab[k]$ with payload $\mpD$ is received %
(for some $k \!\in\! I$), %
then the execution continues as $\mpP_k$, %
with $x_k$ replaced by $\mpD$; if not received, it triggers the exception.
Note that message labels $\mpLab[i]$ are pairwise distinct and
their order is irrelevant, and %
variable $x_i$ is bound with scope $\mpP_i$.

The following two failure handling processes follow a program behaviour of
\Cref{fig:implementation:role:s}.
The \textbf{try-catch} process, $\trycatch{P}{Q}$, consists of
a \emph{try process} $P$ which is ready to communicate with
parallel composed one; and a \emph{catch process} $Q$ which
becomes active when a cancellation happens.
The \textbf{cancel} process, $\mpCancel{\mpC}{\mpP}$, cancels
other processes whose communication channel is $c$.
The \textbf{kill} $\kills{\mpS}$ kills
all processes with session $\mpS$ and generated only at runtime
from a process with errors or $\mpQuestion$-option.

Other syntax is from~\cite{scalasLess2019}.
The \textbf{inaction $\mpNil$} represents a terminated process %
(and is often omitted).
The \textbf{parallel composition $\mpP \mpPar \mpQ$} %
represents two processes that can execute concurrently, %
and potentially communicate.
The \textbf{session restriction $\mpRes{\mpS}{\mpP}$} %
declares a new session $\mpS$ with a scope limited to process $\mpP$.
The linear \textbf{selection} %
and the linear %
\textbf{branching}
can be understood as their affine versions
but without failure handling.

A special selection process
which carries $\chanraise$,
$\mpSel{\mpC}{\roleQ}{\mpLab}{\chanraise}{\mpP}$, is abbreviated
as $\mpRaise{\mpLab}{\mpP}$ and called an \textbf{error} process
to represent a trigger of exception with the label $\mpLab$. We also
write $\mpDaggerBranch{\mpC}{\roleQ}{i \in I}{\mpLab[i]}{x_i}{\mpP[i]}$
and $\mpDaggerSel{\mpC}{\roleQ}{\mpLab}{\mpD}{\mpP}$
to denote either linear or affine branching and selection.

\textbf{Process definition}, $\mpDef{\mpX}{\widetilde{x}}{\mpP}{\mpQ}$ and %
\textbf{process call} $\mpCall{\mpX}{\widetilde{\mpC}}$ model
recursion: the call invokes $\mpX$ %
by expanding it into $\mpP$, %
and replacing its formal parameters with the actual ones.

\paragraph*{Remark (syntax and semantics)}
\AMPST extends~\cite{mostrousAffine2018} to \MPST,
aiming to distil the implementation essence of~\mpstrust (rather
than proposing the minimum \AMPST calculus).
Our \CODE{try-catch} process follows~\cite{mostrousAffine2018}, but
captures more flexible cancellations for arbitrary processes
with affine
branchings/selections (whose semantics follow the implementation
behaviours) and raise processes. Our kill process is generated only at
runtime unlike
\cite{mostrousAffine2018}.
Apart from these differences,
one of the novelties of our formalism is
a combination of session recursions and affinity, which is absent from
the literature~\cite{mostrousAffine2018,fowlerExceptional2019}.
See \S~\ref{sec:related-works} for a detailed comparison including
\cite{harveyMultiparty2021}.



We use $\fv{P}/\fc{P}$ and $\dpv{P}/\fpv{P}$ to denote \emph{free variables}/\emph{channels}
and \emph{bound}/\emph{free process variables} of $P$.
We define a \emph{subject of $P$}, $\sbj{P}$, as:
%$\sbj{\mpQuestionBranch{\mpC}{\roleQ}{i \in
% I}{\mpLab[i]}{x_i}{\mpP[i]}}=\sbj{\mpQuestionSel{\mpC}{\roleQ}{\mpLab}{\mpD}{\mpP}}=
$\sbj{\mpBranch{\mpC}{\roleQ}{i \in I}{\mpLab[i]}{x_i}{\mpP[i]}}=\sbj{\mpSel{\mpC}{\roleQ}{\mpLab}{\mpD}{\mpP}}=\mpC$; $\sbj{\mpCall{\mpX}{\widetilde{\mpC}}}=\mpC_1$
and $\sbj{\mpDefAbbrev{\mpDefD}{\mpP}} = \sbj{\mpP}$;
%\trycatch{\mpP}{\mpQ} = \sbj{\mpP}$;
and others are undefined.
% We define a set of \emph{free subjects of $P$}, $\sbj{P}$, as:
%$\sbj{\mpNil}=\emptyset$;
%$\sbj{\mpP \mpPar \mpQ}= \sbj{\mpP}\cup \sbj{\mpQ}$;
%$\sbj{\mpRes{\mpS}{\mpP}}=\sbj{\mpP}\setminus\{s\}$;
%$\sbj{\mpBranch{\mpC}{\roleQ}{i \in
% I}{\mpLab[i]}{x_i}{\mpP[i]}}=\sbj{\mpSel{\mpC}{\roleQ}{\mpLab}{\mpD}{\mpP}}=\{\mpC\}$; $\sbj{\mpCall{\mpX}{\widetilde{\mpC}}}=\{\widetilde{\mpC}\}$
%and $\sbj{\mpDefAbbrev{\mpDefD}{\mpQ}} = \sbj{\mpQ}$.

\begin{figure*}[t]
\small
  \[
    \begin{array}{rl}
      %\colorbox{ColourShade}{\inferrule{\iruleMPQuestionRedComm}}& %
      %\colorbox{ColourShade}{$\mpQuestionBranch{\mpChanRole{\mpS}{\roleP}}{\roleQ}{i \in I}{%
      %     \mpLab[i]}{x_i}{\mpP[i]}%
      %      \,\mpPar\,%
      %      \mpQuestionSel{\mpChanRole{\mpS}{\roleQ}}{\roleP}{\mpLab[k]}{%
      %        \mpChanRole{\mpSi}{\roleR}%
      %      }{\mpQ}%
      %      \;\;\mpMove\;\;%
      %      \mpP[k]\subst{\mpFmt{x_k}}{\mpChanRole{\mpSi}{\roleR}}%
      %      \,\mpPar\,%
      %      \mpQ%
      %      \quad%
      %      \text{if\, $k \!\in\! I$}$}%
      %      \\[2mm]%
      \colorbox{ColourShade}{\inferrule{\iruleMPRedComm}} & %
      \colorbox{ColourShade}{$\mpEtx_{1}[\mpDaggerBranch{\mpChanRole{\mpS}{\roleP}}{\roleQ}{i \in I}{%
              \mpLab[i]}{x_i}{\mpP[i]}]%
          \,\mpPar\,%
          \mpEtx_{2}[\mpDaggerSel{\mpChanRole{\mpS}{\roleQ}}{\roleP}{\mpLab[k]}{%
              \mpChanRole{\mpSi}{\roleR}%
            }{\mpQ}]%
          \;\;\mpMove\;\;%
          \mpP[k]\subst{\mpFmt{x_k}}{\mpChanRole{\mpSi}{\roleR}}%
          \,\mpPar\,%
          \mpQ%
          \quad%
          \text{if\, $k \!\in\! I$}$}%
      \\[2mm]%
      \colorbox{ColourShade}{\inferrule{\iruleMPRedCat}}  & %
      \colorbox{ColourShade}{$\trycatch{\mpRaise{\mpLab}{P}}{Q}
          \mpMove Q$}
      \quad\quad\quad
      \colorbox{ColourShade}{\inferrule{\iruleMPRedCan}}\
      \colorbox{ColourShade}{$\mpCancel{\mpChanRole{\mpS}{\roleP}}{Q}
          \mpMove \kills{s}\mpPar Q$}
      \\[2mm]%
      \colorbox{ColourShade}{\inferrule{\iruleMPCQSel}}   & %
      \colorbox{ColourShade}{$
          \mpQuestionSel{\mpChanRole{\mpS}{\roleP}}{\roleQ}{\mpLab}{
            \mpChanRole{\mpS'}{\roleR}}{\mpP}
          \mpMove
          \mpSel{\mpChanRole{\mpS}{\roleP}}{\roleQ}{\mpLab}{
            \mpChanRole{\mpS'}{\roleR}}{\mpP}
          \mpPar \kills{\mpS}$}
      % \quad\quad\quad
      \\[2mm]%
      \colorbox{ColourShade}{$\inferrule{\iruleMPCSel}$}  & %
      \colorbox{ColourShade}{$\mpSel{\mpChanRole{\mpS}{\roleP}}{\roleQ}{\mpLab}{
            \mpChanRole{\mpS'}{\roleR}}{\mpP}
          \mpPar \kills{\mpS}
          \mpMove
          \mpP \mpPar \kills{\mpS} \mpPar \kills{\mpS'}$}
      %
      \\[2mm]%
      \colorbox{ColourShade}{$\inferrule{\iruleMPCQBra}$} & %
      \colorbox{ColourShade}{$\mpQuestionBranch{\mpChanRole{\mpS}{\roleP}}{\roleQ}{i \in
            I}{\mpLab[i]}{x_i}{\mpP[i]}%
          \mpMove
          \mpBranch{\mpChanRole{\mpS}{\roleP}}{\roleQ}{i \in
            I}{\mpLab[i]}{x_i}{\mpP[i]}
          \mpPar \kills{\mpS}$}
      \\[2mm]%
      \colorbox{ColourShade}{$\inferrule{\iruleMPCBra}$}  & %
      \colorbox{ColourShade}{$\mpBranch{\mpChanRole{\mpS}{\roleP}}{\roleQ}{i \in
            I}{\mpLab[i]}{x_i}{\mpP[i]} \mpPar \kills{\mpS}%
          \mpMove
          \mpRes{\mpS'}(\mpP[k]\subst{\mpFmt{x_k}}{\mpChanRole{\mpS'}{\roleR}}
          \mpPar \kills{\mpS'})
          \mpPar \kills{\mpS}
          \quad \text{$\mpS'\not\in \fc{P_k}, k\in I$}$}
      \\[2mm]%
      \colorbox{ColourShade}{$\inferrule{\iruleMPCCat}$}  & %
      \colorbox{ColourShade}{$\trycatch{P}{Q} \mpPar \kills{\mpS}
          \mpMove Q \mpPar \kills{\mpS}
          \quad \text{$\mpChanRole{\mpS}{\roleR}=\sbj{P}$ for some $\roleR$}$}
      \\[2mm]%
      \inferrule{\iruleMPRedCall}                         & %
      \mpDef{\mpX}{x_1,\dots,x_n}{\mpP}{(%
        \mpCall{\mpX}{%
          \mpChanRole{\mpS[1]}{\roleP[1]}, \dots,%
          \mpChanRole{\mpS[n]}{\roleP[n]}%
        }%
        \mpPar%
        \mpQ%
        )%
      }%
      \\[2mm]%
                                                          & %
      \qquad%
      \mpMove %
      \mpDef{\mpX}{x_1,..,x_n}{\mpP}{(%
        \mpP\subst{\mpFmt{x_1}}{\mpChanRole{\mpS[1]}{\roleP[1]}}%
        \cdot\cdot
        \subst{\mpFmt{x_n}}{\mpChanRole{\mpS[n]}{\roleP[n]}}%
        \mpPar%
        \mpQ%
        )%
      }%
      \\[2mm]%
      \inferrule{\iruleMPRedCtx}                          & %
      \mpP \mpMove \mpPi%
      \;\;\text{implies}\;\;%
      \mpCtx{}[\mpP] \mpMove \mpCtx{}[\mpPi]
      \quad\quad
      \inferrule{\iruleMPRedSt}\quad
      \mpP \equiv \mpPi \mpMove \mpQi \equiv \mpQ%
      \;\;\text{implies}\;\;%
      \mpP \mpMove \mpQ
      %      \mpP \mpPar \mpQ \mpMove \mpPi \mpPar \mpQ
      %      \;\;\text{and}\;\;%
      %      \mpRes{\mpS}{\mpP} \mpMove \mpRes{\mpS}{\mpPi}
      %      \;\;\text{and}\;\;%
      %\mpDefAbbrev{\mpDefD}{\mpP} \mpMove \mpDefAbbrev{\mpDefD}{\mpPi}%
      %\text{$\{\mpChanRole{\mpS}{\roleR_1},...,\mpChanRole{\mpS}{\roleR_n}\} \supseteq\sbj{P}$}
      %      \\[2mm]%
      %\inferrule{\iruleMPCCat}&%
      %\trycatch{P}{Q} \mpPar
      %\kills{\mpS_1} \mpPar \dots \mpPar \kills{\mpS_n}
      %\mpMove Q \mpPar \kills{\mpS_1} \mpPar \dots \mpPar \kills{\mpS_n}
      %\quad
      %\text{$\{\mpS_1,...,\mpS_n\}\supseteq\fc{P}$}
      %
      %      \inferrule{\iruleMPErrLabel}&%
      %      \mpBranch{\mpChanRole{\mpS}{\roleP}}{\roleQ}{i \in I}{%
      %        \mpLab[i]}{x_i}{\mpP[i]}%
      %      \,\mpPar\,%
      %      \mpSel{\mpChanRole{\mpS}{\roleQ}}{\roleP}{\mpLab}{%
      %        \mpChanRole{\mpSi}{\roleR}%
      %      }{\mpQ}%
      %      \;\;\mpMove\;\;%
      %      \mpErr%
      %      \quad%
      %      \text{if\, $\forall i \!\in\! I: \mpLab[i] \!\neq\! \mpLab$}%
    \end{array}
  \]

\rule{\textwidth}{0.3mm}

\[
      \colorbox{ColourShade}{$\kills{\mpS} \mpPar
          \kills{\mpS}
          \;\equiv\;%
          \kills{\mpS}$}
      \quad%
      \colorbox{ColourShade}{$\mpRes{\mpS}{\kills{\mpS}}%
          \;\equiv\;%
          \mpNil$}%
      \qquad \
      \colorbox{ColourShade}{$\mpDefAbbrev{\mpDefD}{(\trycatch{\mpP}{\mpQ})}%
          \;\equiv\;%
          \trycatch{(\mpDefAbbrev{\mpDefD}{\mpP})}{\mpQ}$}
\]

  \caption{%
    \AMPST $\pi$-calculus reduction (top)
    (we highlight\colorbox{ColourShade}{the new
      rules}from~\cite{scalasLess2019};
and structural congruence rules (the rest are from~\cite{scalasLess2019})
}%
\label{fig:mpst-pi-semantics}%

\end{figure*}

\begin{DEF}[Operational Semantics]\rm
  \label{def:mpst-proc-context}%
  \label{def:mpst-pi-reduction-ctx}%
  \label{def:mpst-pi-semantics}%
  \label{def:mpst-pi-error}%
  A \textbf{try-catch context} $\mpEtx$ is: %
  \;
  %
  %
  \(%
  \mpEtx \,\coloncolonequals\,%
  \trycatch{\mpEtx}{P}%
  \bnfsep%
  \mpEtxHole%
  \)
  and a \textbf{reduction context} $\mpCtx$ is:
  \(\mpCtx \,\coloncolonequals\,
  \mpRes{\mpS}{\mpCtx}%
  \bnfsep%
  \mpDefAbbrev{\mpDefD}{\mpCtx}%
  \bnfsep%
  \mpEtxHole%
  \).
  %
  %
  %  \noindent%
  \ \textbf{Reduction $\mpMove$} %
  is inductively defined %
  in \Cref{fig:mpst-pi-semantics}, which uses the \textbf{structural congruence $\equiv$} %
  \;as the smallest relation between \AMPST processes
  generated in the rules in \Cref{fig:structure}.
  % \iftoggle{techreport}{%
  %   (\Cref{sec:app:mpst})%
  % }{%
  % ~\cite{SY2018TechReport}%
  % } % including $\alpha$-conversion.
  %  We say that \textbf{$\mpP$ has an error}
  %  iff, for some $\mpCtx$,
  %  \,$\mpP \!=\! \mpCtxApp{\mpCtx}{\mpErr}$.
\end{DEF}
We explain each rule highlighting the new rules.
\begin{description}
  \item[Try-Catch] Rule \inferrule{\iruleMPRedComm} is the main
    communication rule between an affine/linear selection and an
    affine/linear branching.
    Linear selections/branching are
    placed in the try position but can interact with affine counterparts.
    Once they interact, processes
    are spawning from a \emph{try-block} and starting communication on parallel
    with other processes.

  \item[Self-Cancellation]
    Rule \inferrule{\iruleMPRedCat}
    models an exceptional behaviour
    raised by exception in Rust.
    Note that the typing rule \inferrule{\iruleMPTryCatch}
    given in \Cref{fig:mpst-rules} ensures that $Q$ is a
    cancel process at the same subject as $\mpRaise{\mpLab}{P}$.
    Rule \inferrule{\iruleMPRedCan} starts broadcasting
    the cancellation message at $s$, generating runtime cancellation
    at $s$.

  \item[Error-Cancellation]
    Rules \inferrule{\iruleMPCQSel} and
    \inferrule{\iruleMPCQBra} model the situations that
    an error handling occurs at the affine selection/branching.
    This might be the case its counterpart has failed (hence
    \inferrule{\iruleMPRedComm} does not happen) or timeout.
    It then triggers the kill process at $s$.

  \item[Cancelling Processes]
    Rule \inferrule{\iruleMPCSel} cancels the selection prefix $s$,
    additionally generating
    the kill process at the delegated channel for all the
    session processes at $s'$ to be eventually cancelled.
    Rule \inferrule{\iruleMPCBra} cancels only one of the branches -- this
    is sufficient enough since all branches contain the same channels
    except $x_i$ (ensured by rule \inferrule{\iruleMPBranch}
    in \Cref{fig:mpst-rules}). After the cancellation, it additionally
    instantiates a fresh name $\mpChanRole{\mpS'}{\roleR}$ to
    $x_k$ into $\mpP[k]$. The generated kill process at $\mpS'$
    kills prefixes at
    $\mpChanRole{\mpS'}{\roleR}$
    in
    $\mpP[k]\subst{\mpFmt{x_k}}{\mpChanRole{\mpS'}{\roleR}}$.

  \item[Cancellation from Other Parties]
    Rule \inferrule{\iruleMPCCat} is prompted to move $\mpQ$
    a cancellation $\kills{s}$. Note that this and rule
    \inferrule{\iruleMPRedCat}
    create \emph{non-determinism} for a \CODE{try-catch} process.

  \item[Other Rules]
    Rules \inferrule{\iruleMPRedCall},
    \inferrule{\iruleMPRedCtx}, and \inferrule{\iruleMPRedSt} are standard from~\cite{scalasLess2019}. In \Cref{fig:structure},
    the first two new rules are for garbage collections of
    kill processes. The third new rule allows
    a try process to contain free process variables and
    infinite session interactions (using \inferrule{\iruleMPRedCtx}).
\end{description}

%\begin{example}{Reductions}
%  \label{ex:reduction}
%  Assume $k \in I$.
%Note that a process might be completed,
%or cancelled in many ways. For example, the following process might
%complete to $

%\centerline{
%    $\begin{array}{ll}
%             & \trycatch{\{\mpSel{\mpChanRole{\mpS}{\roleQ}}{\roleP}{\mpLab[1]}{ %
%          \mpChanRole{\mpSi}{\roleR}%
%        }{
%          \mpChanRole{\mpS}{\roleQ}[\roleP]\mpLab[3](x_3).\mpNil}\}}{\{\mpCancel{\mpChanRole{\mpS}{\roleQ}}
%      {\mpChanRole{\mpS}{\roleQ}[\roleP]\mpLab[3](x_3).\mpNil}\}}                \\
%      \mpPar &
%      \mpQuestion\mpChanRole{\mpS}{\roleP}[\roleQ]({\mpLab[1]}(x_1).
%      \mpQuestionSel{\mpChanRole{\mpS}{\roleP}}{\roleQ}{\mpLab[3]}{x_1}{}
%      \ \mpFmt{+}
%      \ {\mpLab[2]}(x_2).\mpNil)
%    \end{array}
%$}

\subsection{Affine multiparty session typing system}\label{sec:AMPST}
\label{subsec:types}
\myparagraph{Global and local types}
The syntax of types is unchanged from the original system~\cite{scalasLess2019}.
We follow~\cite{scalasLess2019} which is the most widely used syntax in the
literature.
A \emph{global type}, written $\gtG,\gtG',..$,
describes the whole
conversation scenario of a multiparty session as a type signature, and
a {\em local type}, written by $\stS,\stS', \dots$.
% {\em Sorts} $\BT,\BT', \dots$ are associated to values (base types). {\em Payload types} $\UT,\UT', \dots$
% consist of sort types or closed local types, ranged over by $T$.
The syntax of types is given as:

\begin{restatable}[Global types]{DEF}{defMPSTGlobalTypes}\rm
  The syntax of a \textbf{global type $\gtG$} is:%

  \smallskip%
  \centerline{%
    \(%
    \gtG%
    \,\coloncolonequals\,%
    \gtComm{\roleP}{\roleQ}{i \in I}{\gtLab[i]}{\stS[i]}{\gtG[i]}%
    \bnfsep%
    \gtRec{\gtRecVar}{\gtG}%
    \bnfsep%
    \gtRecVar%
    \bnfsep%
    \gtEnd%
    \)%
    \qquad%
    \text{%
      with %
      $\roleP \!\neq\! \roleQ$, %
      \;$I \!\neq\! \emptyset$, %
      \;and\; $\forall i \!\in\! I: \fv{\stS[i]} = \emptyset$%
    }%
  }%
\end{restatable}
\begin{restatable}[Local types]{DEF}{defMPSTLocalTypes}\rm
  The syntax of \textbf{local types} %
  %
  is:

  \smallskip%
  \centerline{\(%
    \textstyle%
    \stS, \stT%
    \,\coloncolonequals\,%
    \stExtSum{\roleP}{i \in I}{\stChoice{\stLab[i]}{\stS[i]} \stSeq \stSi[i]}%
    \bnfsep%
    \stIntSum{\roleP}{i \in I}{\stChoice{\stLab[i]}{\stS[i]} \stSeq \stSi[i]}%
    \bnfsep%
    \stEnd%
    \bnfsep%
    \stRec{\stRecVar}{\stS}%
    \bnfsep%
    \stRecVar
    \quad%
    \text{with $I \!\neq\! \emptyset$,
      and $\stLab[i]$ pairwise distinct}%
    \)}%
  \smallskip%

  \noindent%
  %
  %
  %
  %
  %
  %
  Types must be closed, %
  and recursion variables to be guarded.
\end{restatable}

$\stLab\in \ASigma$ corresponds to the usual message labels in the session type
theory.
% We omit the carried types from the syntax in this
% paper, as we are not directly concerned with typing processes.
Global branching type
$\gtComm{\roleP}{\roleQ}{i \in I}{\gtLab[i]}{\stS[i]}{\gtG[i]}$
states that participant $\roleP$ can
send a message with one of the $\gtLab[i]$ labels and a {\em message payload type} $\stS[i]$
to the participant $\roleQ$ and that interaction
described in $\gtG[i]$ follows.
We require $\roleP\neq\roleQ$ to prevent self-sent messages and
$\gtLab[i]\not= \gtLab[k]$ for all $i\not =k\in J$. Recursive types
$\gtRec{\gtRecVar}{\gtG}$ are for recursive protocols,
assuming those type variables ($\gtRecVar, \gtRecVar', \dots$) are
guarded in the
standard way, \ie they only occur under branching.
Type $\gtEnd$ represents session termination (often omitted).
We write\; $\roleP \in \gtRoles{\gtG}$ %
\;(or simply $\roleP \!\in\! \gtG$) \;iff, for some $\roleQ$, %
either $\gtFmt{\roleP {\to} \roleQ}$ %
or $\gtFmt{\roleQ {\to} \roleP}$ %
occurs in $\gtG$.
The function $\id(\gtG)$ gives the participants of $\gtG$.

For local types, the {\em branching type}
$\stExtSum{\roleP}{i \in I}{\stChoice{\stLab[i]}{\stS[i]} \stSeq \stSi[i]}$
specifies the reception of a message from
$\roleP$ with a label among the $\stLab[i]$ and a payload $\stS[i]$. The {\em selection type}
$\stIntSum{\roleP}{i \in I}{\stChoice{\stLab[i]}{\stS[i]} \stSeq \stSi[i]}$
is its dual. The remaining type
constructors are as for global types.
We say a type is {\em guarded} if it is neither a recursive type nor a type variable.
% When branching is a singleton, we write
%$\TO{p}{p'}:\lab(\UT);{G'}$ for global, and $\LSENDO{\pp}{\lab}{\UT}{\T}$ or $\LRECVO{\pp}{\lab}{\UT}{\T}$ for local.

\myparagraph{Projection}
The relation between global and local types is formalised by
projection~\cite{coppoGlobal2016,hondaMultiparty2008}.

\begin{restatable}[Projection]{DEF}{defMPSTProjection}\rm
  \label{def:projection}
  The
    {\em projection of $\gtG$ onto
      $\roleP$} (written $\gtProj{\gtG}{\roleP}$)
  is defined as:%\\[1mm]

  \smallskip%
  \centerline{\(%
    \small%
    \begin{array}{c}
      \gtProj{\left(%
        \gtComm{\roleQ}{\roleR}{i \in I}{\gtLab[i]}{\stS[i]}{\gtG[i]}%
        \right)}{\roleP}%
      \;=\;%
      \left\{%
      \begin{array}{@{\hskip 0.5mm}l@{\hskip 5mm}l@{}}
        \stIntSum{\roleR}{i \in I}{%
          \stChoice{\stLab[i]}{\stS[i]} \stSeq (\gtProj{\gtG[i]}{\roleP})%
        }%
         & \text{\footnotesize %
          if\, $\roleP = \roleQ$}%
        \\%
        \stExtSum{\roleQ}{i \in I}{%
          \stChoice{\stLab[i]}{\stS[i]} \stSeq (\gtProj{\gtG[i]}{\roleP})%
        }%
         & \text{\footnotesize %
          if\, $\roleP = \roleR$}%
        \\%
        \stMerge{i \in I}{\gtProj{\gtG[i]}{\roleP}}%
         & \text{\footnotesize %
          if\, $\roleQ \neq \roleP \neq \roleR$}%
      \end{array}
      \right.
      % \quad
      \\[6mm]%
      \begin{array}{rcl}
        \gtProj{(\gtRec{\gtRecVar}{\gtG})}{\roleP}%
         & = & %
        \left\{%
        \begin{array}{@{\hskip 0.5mm}l@{\hskip 5mm}l@{}}
          \stRec{\stRecVar}{(\gtProj{\gtG}{\roleP})}%
           & %
          \text{\footnotesize%
            if\, $\gtProj{\gtG}{\roleP} \neq \stRecVari$ ($\forall \stRecVari$)%
          }%
\\
          \stEnd%
           & %
          \text{\footnotesize%
            otherwise}
        \end{array}
        \right.%
\qquad
        %    \begin{array}{@{}r@{\hskip 1mm}c@{\hskip 1mm}l@{}}
        \gtProj{\gtRecVar}{\roleP}%
          = %
        \stRecVar%
\qquad
        \gtProj{\gtEnd}{\roleP}%
          =  %
        \stEnd%
        %    \end{array}
      \end{array}
    \end{array}
    \)}%
  \smallskip%

  \noindent%
  For projection of branching, we introduce a merge
  operator along the lines of~\cite{denielouDynamic2011},
  written $\stS \stBinMerge \stS'$, ensuring
  that if the locally observable behaviour of the local type is
  dependent of the chosen branch then it is identifiable via a unique
  choice/branching label.

  The \emph{merging operation} $\stBinMerge{}{}$ is defined as a partial commutative
  operator over two types such that:

  \smallskip%
  \centerline{\(%
    \small%
    \begin{array}{c}%
      \textstyle%
      \stExtSum{\roleP}{i \in I}{\stChoice{\stLab[i]}{\stS[i]} \stSeq \stSi[i]}%
      \,\stBinMerge\,%
      \stExtSum{\roleP}{\!j \in J}{\stChoice{\stLab[j]}{\stS[\!j]} \stSeq \stTi[j]}%
      \;=\;%
      \stExtSum{\roleP}{k \in I \cap J}{\stChoice{\stLab[k]}{\stS[k]} \stSeq%
        (\stSi[k] \!\stBinMerge\! \stTi[k])%
      }%
      \stExtC%
      \stExtSum{\roleP}{i \in I \setminus J}{\stChoice{\stLab[i]}{\stS[i]} \stSeq \stSi[i]}%
      \stExtC%
      \stExtSum{\roleP}{\!j \in J \setminus I}{\stChoice{\stLab[j]}{\stS[\!j]} \stSeq \stTi[j]}%
      \\[1mm]%
      \stIntSum{\roleP}{i \in I}{\stChoice{\stLab[i]}{\stS[i]} \stSeq \stSi[i]}%
      \,\stBinMerge\,%
      \stIntSum{\roleP}{i \in I}{\stChoice{\stLab[i]}{\stS[i]} \stSeq \stSi[i]}%
      \;=\;%
      \stIntSum{\roleP}{i \in I}{\stChoice{\stLab[i]}{\stS[i]} \stSeq \stSi[i]}%
%      \\[1mm]%
      \qquad%
      \stRec{\stRecVar}{\stS} \,\stBinMerge\, \stRec{\stRecVar}{\stT}%
      \;=\;%
      \stRec{\stRecVar}{(\stS \stBinMerge \stT)}%
      \qquad%
%      \stRecVar \,\stBinMerge\, \stRecVar%
      \stT \,\stBinMerge\, \stT%
      \;=\;%
      \stT%
%      \qquad%
%      \stEnd \,\stBinMerge\, \stEnd%
%      \;=\;%
%      \stEnd%
    \end{array}
    \)}%
\end{restatable}
\noindent As an example of projection, consider
$\gtRec{\gtRecVar}{\gtCommRaw{\roleAlice}{\roleBob}{
          \gtCommChoiceSmall{a}{}{
            \gtCommRaw{\roleBob}{\roleCarol}{
              \gtCommChoiceSmall{b}{}{
                \gtCommRaw{\roleAlice}{\roleCarol}{\gtCommChoiceSmall{c}{}{
                    \gtRecVar}}}}},
          \gtCommChoiceSmall{d}{}{
            \gtCommRaw{\roleBob}{\roleCarol}{
              \gtCommChoiceSmall{e}{}{
                \gtCommRaw{\roleAlice}{\roleCarol}{
                  \gtCommChoiceSmall{f}{}{\gtEnd}}}}}}}$.
Then $\roleCarol$'s local type is given by:
$\stRec{\stRecVar}{
    \stExtSum{\roleBob}{}{\{
      \stChoice{\stLabFmt{b}}{} \stSeq
      \stExtSum{\roleAlice}{}{\stLabFmt{c}} \stSeq \stRecVar,
      \stChoice{\stLabFmt{e}}{} \stSeq
      \stExtSum{\roleAlice}{}{\stLabFmt{f}} \stSeq \stEnd
      \}}
  }$.
We say that $G$ is {\em well-formed} if for all $\roleP\in \PSet$,
$\gtProj{\gtG}{\roleP}$ is defined.
We also use the standard \emph{multiparty session subtyping relation} from
\cite{ghilezanPrecise2019,dezaniCiancagliniPrecise2015}
%.\footnote{%
%  \label{footnote:inverted-subt}%
%  For convenience, we use the ``channel-oriented'' order %
%  of~\citeN{gaySubtyping2005,scalasLinear2017} for our subtyping relation.
%  For a comparison with
%  ``process-oriented'' subtyping of~\citeN{ghilezanPrecise2019},
%  see~\cite{gaySubtyping2016}.} %
%Intuitively, a type $\stS$ is smaller than $\stS'$ %
%when $\stS$ is ``less demanding'' than $\stS'$,
%\ie when $\stS$ imposes to support less external choices
%and allows performing more internal choices.
%Session subtyping is used in the type system %
%to augment its flexibility.
%
\begin{DEF}[Subtyping]\rm
  \label{def:session:subtyping}
  The subtyping relation $\stSub$ is \emph{co}inductively defined as:
  \smallskip%

  \centerline{\(%
    \begin{array}{c}%
      \cinference[\iruleSubBranch]{
        \forall i \in I%
       & %
        \stS[i] \stSub \stT[i]%
       & %
        \stSi[i] \stSub \stTi[i]%
      }{%
        \stExtSum{\roleP}{i \in I}{\stChoice{\stLab[i]}{\stS[i]} \stSeq \stSi[i]}%
        \stSub%
        \stExtSum{\roleP}{i \in I \cup J}{\stChoice{\stLab[i]}{\stT[i]} \stSeq \stTi[i]}%
      }%
      \qquad%
      \cinference[\iruleSubSel]{
        \forall i \in I%
       & %
        \stT[i] \stSub \stS[i]%
       & %
        \stSi[i] \stSub \stTi[i]%
      }{%
        \stIntSum{\roleP}{i \in I \cup J}{\stChoice{\stLab[i]}{\stS[i]} \stSeq \stSi[i]}%
        \stSub%
        \stIntSum{\roleP}{i \in I}{\stChoice{\stLab[i]}{\stT[i]} \stSeq \stTi[i]}%
      }%
      \\[2mm]%
      \cinference[\iruleSubEnd]{%
        \phantom{X}%
      }{%
        \stEnd \stSub \stEnd%
      }%
      \qquad%
      \cinference[\iruleSubRecL]{%
        \stS\subst{\stRecVar}{\stRec{\stRecVar}{\stS}} \stSub \stT%
      }{%
        \stRec{\stRecVar}{\stS} \stSub \stT%
      }%
      \qquad%
      \cinference[\iruleSubRecR]{%
        \stS \stSub \stT\subst{\stRecVar}{\stRec{\stRecVar}{\stT}}%
      }{%
        \stS \stSub \stRec{\stRecVar}{\stT}
      }%
    \end{array}
    \)}%
\end{DEF}
We define typing contexts which are used to define properties of
type-level behaviours.
\begin{DEF}[Typing Contexts]\rm%
  \label{def:mpst-env}%
  \label{def:mpst-env-closed}%
  \label{def:mpst-env-comp}%
  \label{def:mpst-env-subtype}%
  $\mpEnv$ denotes a partial mapping %
  from process variables to $n$-tuples of types, %
  and $\stEnv$ denotes a partial mapping %
  from channels to types, %
  defined as:%

  \smallskip%
  \centerline{\(%
    \mpEnv%
    \;\;\coloncolonequals\;\;%
    \mpEnvEmpty%
    \bnfsep%
    \mpEnv \mpEnvComp\, \mpEnvMap{\mpX}{\stS[1],\dots,\stS[n]}%
    \quad\quad
    \stEnv%
    \,\coloncolonequals\,%
    \stEnvEmpty%
    \bnfsep%
    \stEnv \stEnvComp \stEnvMap{c}{\stS}%
    %  \bnfsep%
    %  \stEnv \stEnvComp \stEnvMap{\mpChanRole{\mpS}{\roleP}}{\stS}%
    \)}%
  \smallskip%

  \noindent%
  The \,\emph{composition} $\stEnv[1] \stEnvComp \stEnv[2]$\,
  is defined iff $\dom{\stEnv[1]} \cap \dom{\stEnv[2]} = \emptyset$.
  %

  \noindent%
  We write\; %
  $\mpS \!\not\in\! \stEnv$ %
  \;iff\; %
  $\forall \roleP: \mpChanRole{\mpS}{\roleP} \!\not\in\! \dom{\stEnv}$ %
  (\ie session $\mpS$ does not occur in $\stEnv$).%

  \noindent%
  We write\; %
  $\dom{\stEnv} \!=\! \setenum{\mpS}$ %
  \;iff\; %
  $\forall \mpC \!\in\! \dom{\stEnv}$ there is $\roleP$ such that %
  $\mpC \!=\! \mpChanRole{\mpS}{\roleP}$ %
  (\ie $\stEnv$ only contains session $\mpS$).%
  %

  \noindent%
  We write %
  $\stEnv \!\stSub\! \stEnvi$ %
  iff %
  $\dom{\stEnv} \!=\! \dom{\stEnvi}$ %
  and %
  $\forall \mpC \!\in\! \dom{\stEnv}{:}\,%
    \stEnvApp{\stEnv}{\mpC} \!\stSub\! \stEnvApp{\stEnvi}{\mpC}$.%
\end{DEF}

\begin{DEF}[Typing Context Safety]\rm
  \label{def:mpst-env-safe}%
  $\predP$ is a \emph{safety property} of typing contexts %
  iff: %

  \begin{tabular}{r@{\hskip 2mm}l}
    \inferrule{\iruleSafeComm}%
     & %
    $\predPApp{%
        \stEnv \stEnvComp\,%
        \stEnvMap{%
          \mpChanRole{\mpS}{\roleP}%
        }{%
          \stIntSum{\roleQ}{i \in I}{\stChoice{\stLab[i]}{\stS[i]} \stSeq \stSi[i]}%
        }%
        \stEnvComp\,%
        \stEnvMap{%
          \mpChanRole{\mpS}{\roleQ}%
        }{%
          \stExtSum{\roleP}{j \in J}{\stChoice{\stLab[j]}{\stT[j]} \stSeq \stTi[j]}%
        }%
      }$%
    \;\;implies\;\; %
    $I \!\subseteq\! J$\,, %
    \,and\, %
    $\forall i \!\in\! I: \stS[i] \!\stSub\! \stT[i]$;
    \\%
    \inferrule{\iruleSafeRec}%
     & %
    $\predPApp{%
        \stEnv \stEnvComp\, \stEnvMap{%
          \mpChanRole{\mpS}{\roleP}%
        }{%
          \stRec{\stRecVar}{\stS}%
        } %
      }$ %
    \;\;implies\;\; %
    $\predPApp{%
        \stEnv \stEnvComp\, \stEnvMap{%
          \mpChanRole{\mpS}{\roleP}%
        }{%
          \stS\subst{\stRecVar}{\stRec{\stRecVar}{\stS}}%
        }%
      }$;
    \\%
    \inferrule{\iruleSafeMove}%
     & %
    $\predPApp{\stEnv}$ %
    \;and\; $\stEnv \stEnvMove \stEnvi$ %
    \;\;implies\;\; %
    $\predPApp{\stEnvi}$.
  \end{tabular}

  \noindent%
  We say \emph{$\stEnv$ is safe}, %
  written $\stEnvSafeP{\stEnv}$, %
  if $\predPApp{\stEnv}$ %
  for some safety property $\predP$.
  % We define $\stEnvSafePred$ as the largest safety property, %
  % \ie the union of all safety properties.
\end{DEF}

\begin{restatable}[]{DEF}{defMPSTTyping}\rm
  The typing judgements for processes has two forms:
  \begin{equation}
    \label{eq:typing-judgement}%
    \stJudgeTry{\mpEnv}{\stEnv}{\mpP}%
    \  \text{and} \
    \stJudge{\mpEnv}{\stEnv}{\mpP}%
    \
    \text{%
      (with $\mpEnv$/$\stEnv$ omitted when empty)%
    }%
  \end{equation}
  and are defined by the typing rules in \Cref{fig:mpst-rules}.
  The first judgement types try processes
  that ensures that
  only (infinite) prefixed processes
  to be placed in the try position $[\ ]$ in $\trycatch{[\ ]}{Q}$.
  The second judgement types all forms of processes.
  For convenience, we type-annotate %
  channels bound by process definitions and restrictions.
\end{restatable}

\begin{figure}[t]
%  \hspace{-5mm}%
\small
%  \scalebox{0.9}{%
%\begin{minipage}{\textwidth}
\[
\begin{array}{c}
          \inference[\iruleMPX]{%
            \mpEnvApp{\mpEnv}{X} = \stFmt{\stS[1],\dots,\stS[n]}%
          }{%
            \mpEnvEntails{\mpEnv}{X}{\stS[1],\dots,\stS[n]}%
          }%
          \quad%
          \inference[\colorbox{ColourShade}{\iruleMPRaise}]{%
            %\stS \stSub \stSi \quad \mpC\not=\chanraise%
          }{%
            \colorbox{ColourShade}{$\stEnvEntails{\stEnvMap{\chanraise}{\stEnd}}{\chanraise}{\stEnd}$}%
          }%
          \quad
          \inference[\iruleMPSub]{%
            \stS \stSub \stSi \quad \mpC\not=\chanraise%
          }{%
            \stEnvEntails{\stEnvMap{\mpC}{\stS}}{\mpC}{\stSi}%
          }%
\\[3mm]
          \inference[\iruleMPEnd]{%
            \forall i \in 1..n%
           &                             %
            \stEnvEntails{\stEnvMap{\mpC[i]}{\stS[i]}}{%
              \mpC[i]%
            }{%
              \stEnd%
            }%
          }{%
            \stEnvEndP{%
              \stEnvMap{\mpC[1]}{\stS[1]}%
              \stEnvComp \dots \stEnvComp%
              \stEnvMap{\mpC[n]}{\stS[n]}%
            }%
          }%
          \quad
          \inference[\colorbox{ColourShade}{\iruleMPPromote}]{%
            \colorbox{ColourShade}{$\stJudgeTry{\mpEnv}{%
                  \stEnv%
                }{%
                  \mpP
                }$}%
          }{%
            \stJudge{\mpEnv}{%
              \stEnv%
            }{%
              \mpP
            }%
          }%
          \quad
          \inference[\iruleMPNil]{%
            \stEnvEndP{\stEnv}%
            %
            %
            %
          }{%
            \colorbox{ColourShade}{$\stJudgeTry{\mpEnv}{\stEnv}{\mpNil}$}%
          }%
\quad
          \inference[\iruleMPPar]{%
            \stJudge{\mpEnv}{%
              \stEnv[1]%
            }{%
              \mpP[1]%
            }%
            \qquad%
            \stJudge{\mpEnv}{%
              \stEnv[2]%
            }{%
              \mpP[2]%
            }%
          }{%
            \stJudge{\mpEnv}{%
              \stEnv[1] \stEnvComp \stEnv[2]%
            }{%
              \mpP[1] \mpPar \mpP[2]%
            }%
          }%
          \\[3mm]
          \inference[\iruleMPBranch]{%
            \stEnvEntails{\stEnv[1]}{\mpC}{%
              \stExtSum{\roleQ}{i \in I}{\stChoice{\stLab[i]}{\stS[i]} \stSeq \stSi[i]}%
            }%
           &                             %
            \forall i \!\in\! I%
           &                             %
            \stJudge{\mpEnv}{%
              \stEnv \stEnvComp%
              \stEnvMap{y_i}{\stS[i]} \stEnvComp%
              \stEnvMap{\mpC}{\stSi[i]}%
            }{%
              \mpP[i]%
            }%
          }{%
            \colorbox{ColourShade}{$\stJudgeTry{\mpEnv}{%
                  \stEnv \stEnvComp \stEnv[1]%
                }{%
                  \mpBranch{\mpC}{\roleQ}{i \in I}{\mpLab[i]}{y_i}{\mpP[i]}%
                }$}%
          }%
\quad
          \inference[\iruleMPSel]{%
            \stEnvEntails{\stEnv[1]}{\mpC}{%
              \stIntSum{\roleQ}{}{\stChoice{\stLab}{\stS} \stSeq \stSi}%
            }%
           &                             %
            \stEnvEntails{\stEnv[2]}{\mpD}{\stS}%
           &                             %
            \stJudge{\mpEnv}{%
              \stEnv \stEnvComp \stEnvMap{\mpC}{\stSi}%
            }{%
              \mpP%
            }%
          }{%
            \colorbox{ColourShade}{$\stJudgeTry{\mpEnv}{%
                  \stEnv \stEnvComp \stEnv[1] \stEnvComp \stEnv[2]%
                }{%
                  \mpSel{\mpC}{\roleQ}{\mpLab}{\mpD}{\mpP}%
                }$}%
          }%
          \quad\quad
          \\[3mm]
          \inference[\colorbox{ColourShade}{\iruleMPQBranch}]{%
            \stEnvEntails{\stEnv[1]}{\mpC}{%
              \stExtSum{\roleQ}{i \in I}{\stChoice{\stLab[i]}{\stS[i]} \stSeq \stSi[i]}%
            }%
           &                             %
            \forall i \!\in\! I%
           &                             %
            \stJudge{\mpEnv}{%
              \stEnv \stEnvComp%
              \stEnvMap{y_i}{\stS[i]} \stEnvComp%
              \stEnvMap{\mpC}{\stSi[i]}%
            }{%
              \mpP[i]%
            }%
          }{%
            \colorbox{ColourShade}{$\stJudge{\mpEnv}{%
                  \stEnv \stEnvComp \stEnv[1]%
                }{%
                  \mpQuestionBranch{\mpC}{\roleQ}{i \in I}{\mpLab[i]}{y_i}{\mpP[i]}%
                }$}%
          }%
          \quad
          \inference[\iruleMPQSel]{%
            \stEnvEntails{\stEnv[1]}{\mpC}{%
              \stIntSum{\roleQ}{}{\stChoice{\stLab}{\stS} \stSeq \stSi}%
            }%
           &                             %
            \stEnvEntails{\stEnv[2]}{\mpD}{\stS}%
           &                             %
            \stJudge{\mpEnv}{%
              \stEnv \stEnvComp \stEnvMap{\mpC}{\stSi}%
            }{%
              \mpP%
            }%
          }{%
            \colorbox{ColourShade}{$\stJudge{\mpEnv}{%
                  \stEnv \stEnvComp \stEnv[1] \stEnvComp \stEnv[2]%
                }{%
                  \mpQuestionSel{\mpC}{\roleQ}{\mpLab}{\mpD}{\mpP}%
                }$}%
          }%
          \\[3mm]
          \inference[\colorbox{ColourShade}{\iruleMPTryCatch}]{%
            \colorbox{ColourShade}{$\stJudgeTry{\mpEnv}{%
                  \stEnv\stEnvComp \stEnvMap{c}{\stS}%
                }{%
                  \mpP%
                }$}%
            \qquad%
            \colorbox{ColourShade}{$\sbj{P}=c$}
            \qquad%
            \colorbox{ColourShade}{$\stJudge{}{%
                  \stEnv%
                }{%
                  {\mpQ}%
                }$}%
          }{%
            \colorbox{ColourShade}{$\stJudge{\mpEnv}{\stEnv\stEnvComp \stEnvMap{c}{\stS}}
                {%
                  \trycatch{P}{\mpCancel{c}{Q}}
                }%
              $}}%
\quad
          \inference[\colorbox{ColourShade}{\iruleMPKills}]{%
            \colorbox{ColourShade}{$\stEnvEndP{\stEnv}$}%
            \quad \colorbox{ColourShade}{$0\leq n$}
            %
            %
            %
          }{%
            \colorbox{ColourShade}{$\stJudge{\mpEnv}{\stEnv \stEnvComp
                  \stEnvMap{\mpChanRole{\mpS}{\roleP_1}}{\stS[1]}\stEnvComp
                  \stEnvMap{\mpChanRole{\mpS}{\roleP_2}}{\stS[2]}\stEnvComp
                  \dots
                  \stEnvComp
                  \stEnvMap{\mpChanRole{\mpS}{\roleP_n}}{\stS[n]}
                }
                {
                  \kills{s}
                }$}%
          }%
          \\[3mm]
          \inference[\colorbox{ColourShade}{\iruleMPCancel}]{%
            \colorbox{ColourShade}{$\stJudge{\mpEnv}{%
                  \stEnv%
                }{%
                  {\mpQ}%
                }$}%
            \quad \colorbox{ColourShade}{$1\leq n$}
            %
            %
            %
          }{%
            \colorbox{ColourShade}{$\stJudge{\mpEnv}{\stEnv \stEnvComp
                  \stEnvMap{\mpChanRole{\mpS}{\roleP_1}}{\stS[1]}\stEnvComp
                  \stEnvMap{\mpChanRole{\mpS}{\roleP_2}}{\stS[2]}\stEnvComp
                  \dots
                  \stEnvComp
                  \stEnvMap{\mpChanRole{\mpS}{\roleP_n}}{\stS[n]}
                }
                {
                  \mpCancel{\mpChanRole{\mpS}{\roleR}}{Q}
                }$}%
          }%

\\[3mm]
          \inference[\iruleMPDef]{%
            %
            \stJudge{%
              \mpEnv \mpEnvComp%
              \mpEnvMap{\mpX}{\stS[1],\dots,\stS[n]}%
            }{%
              \stEnvMap{x_1}{\stS[1]}%
              \stEnvComp \dots \stEnvComp%
              \stEnvMap{x_n}{\stS[n]}%
            }{%
              \mpP%
            }%
            \qquad%
            \stJudge{%
              \mpEnv \mpEnvComp%
              \mpEnvMap{\mpX}{\stS[1],\dots,\stS[n]}%
            }{%
              \stEnv%
            }{%
              \mpQ%
            }%
            %
          }{%
            \stJudge{\mpEnv}{%
              \stEnv%
            }{%
              \mpDef{\mpX}{%
                \stEnvMap{x_1}{\stS[1]},%
                \dots,%
                \stEnvMap{x_n}{\stS[n]}%
              }{\mpP}{\mpQ}%
            }%
          }%
          \\[3mm]%
          \inference[\colorbox{ColourShade}{\iruleMPDefTry}]{%
            %
            \colorbox{ColourShade}{$\stJudgeTry{%
                  \mpEnv \mpEnvComp%
                  \mpEnvMap{\mpX}{\stS[1],\dots,\stS[n]}%
                }{%
                  \stEnvMap{x_1}{\stS[1]}%
                  \stEnvComp \dots \stEnvComp%
                  \stEnvMap{x_n}{\stS[n]}%
                }{%
                  \mpP%
                }$}%
            \qquad%
            \colorbox{ColourShade}{$\stJudgeTry{%
                  \mpEnv \mpEnvComp%
                  \mpEnvMap{\mpX}{\stS[1],\dots,\stS[n]}%
                }{%
                  \stEnv%
                }{%
                  \mpQ%
                }$}%
            \qquad%
            \colorbox{ColourShade}{${\forall i \in 2..n%
                    \ S_i=\stEnd}$}
          }{%
            \colorbox{ColourShade}{$\stJudgeTry{\mpEnv}{%
                  \stEnv%
                }{%
                  \mpDef{\mpX}{%
                    \stEnvMap{x_1}{\stS[1]},%
                    \dots,%
                    \stEnvMap{x_n}{\stS[n]}%
                  }{\mpP}{\mpQ}%
                }$}%
          }%
          \\[3mm]%
          \inference[\iruleMPCall]{%
            %
            \mpEnvEntails{\mpEnv}{X}{%
              \stS[1],\dots,\stS[n]%
            }%
           &                             %
            \stEnvEndP{\stEnv[0]}%
           &                             %
            \forall i \in 1..n%
           &                             %
            \stEnvEntails{\stEnv[i]}{\mpC[i]}{\stS[i]}%
            %
          }{%
            \stJudge{\mpEnv}{%
              \stEnv[0] \stEnvComp%
              \stEnv[1] \stEnvComp \dots \stEnvComp \stEnv[n]%
            }{%
              \mpCall{\mpX}{\mpC[1],\dots,\mpC[n]}%
            }%
          }%
          \\[3mm]
          \inference[\colorbox{ColourShade}{\iruleMPCallTry}]{%
            %
            \mpEnvEntails{\mpEnv}{X}{%
              \stS[1],\dots,\stS[n]%
            }%
           &                             %
            {\colorbox{ColourShade}{$\stEnvEndP{\stEnv[0],\stEnv[2],...,\stEnv[n]}$}}%
           &                             %
            \forall i \in 1..n%
           &                             %
            \stEnvEntails{\stEnv[i]}{\mpC[i]}{\stS[i]}%
            %
          }{%
            \colorbox{ColourShade}{$\stJudgeTry{\mpEnv}{%
                  \stEnv[0] \stEnvComp%
                  \stEnv[1] \stEnvComp \dots \stEnvComp \stEnv[n]%
                }{%
                  \mpCall{\mpX}{\mpC[1],\dots,\mpC[n]}%
                }$}%
          }%
          \\[3mm]
          % \begin{array}{@{}c@{}}
          %     \inference[\iruleMPInit]{%
          %       \stEnv_i = \setenum{%
          %         \stEnvMap{\mpChanRole{\mpS_i}{\roleP}}{\gtProj{\gtG_i}{\roleP}}%
          %       }_{\roleP \in \gtRoles{\gtG_i}}%
          %      \qquad%
          %      \mpS \not\in \stEnv%
          %       \qquad%
          % \stEnv = \stEnv_1,\dots,\stEnv_n%
          % \quad
          %       \stJudge{}{\stEnv}{%
          %       }{%
          %         \mpP%
          %       }%
          %     }{%
          %       \stJudge{}{}{%
          %        \mpRes{\stEnvMap{\mpS_i}{\stEnv_i}}
          %      {\mpP}%
          %       }%
          %     }%
          % \end{array}\\[3mm]
          \begin{array}{@{}c@{}}
            \inference[\iruleMPInit]{%
              \stEnvi = \setenum{%
                \stEnvMap{\mpChanRole{\mpS}{\roleP}}{\gtProj{\gtG}{\roleP}}%
              }_{\roleP \in \gtRoles{\gtG}}%
              %      \qquad%
              %      \mpS \not\in \stEnv%
              \quad
              \stJudge{\Theta}{\stEnv \stEnvComp \stEnvi}{%
              }{%
                \mpP%
              }%
            }{%
              \stJudge{\Theta}{\stEnv}{%
                \mpRes{\stEnvMap{\mpS}{\stEnvi}}
                {\mpP}%
              }%
            }%
          \end{array}\quad%\\[3mm]
          \begin{array}{@{}c@{}}
            \inference[\iruleMPSafeRes]{%
              %
              %
              %
              \stEnvi = \setenum{%
                \stEnvMap{\mpChanRole{\mpS}{\roleP}}{\stS[\roleP]}%
              }_{\roleP \in I}%
              \quad%
              \mpS \not\in \stEnv%
              \quad%
              \stEnvSafeP{\stEnvi}%
              \quad%
              \stJudge{\mpEnv}{%
                \stEnv \stEnvComp \stEnvi%
              }{%
                \mpP%
              }%
            }{%
              \stJudge{\mpEnv}{%
                \stEnv%
              }{%
                \mpRes{\stEnvMap{\mpS}{\stEnvi}}\mpP%
              }%
            }%
          \end{array} \\[3mm]
        \end{array}
      \]
%    \end{minipage}
%  }%
  %
  \caption{%
    Multiparty session typing rules.
    We highlight \colorbox{ColourShade}{the new rules} from~\cite{scalasLess2019}.
    %    Rule \inferrule{\iruleMPResProp} %
    %    for session restriction %
    %    is discussed in \Cref{sec:towards-subj-red}.
  }%
  \Description[
    Multiparty session typing rules.
    We highlight \colorbox{ColourShade}{the new rules} from~\cite{scalasLess2019}.
  ]{
    Multiparty session typing rules.
    We highlight \colorbox{ColourShade}{the new rules} from~\cite{scalasLess2019}.
  }%
  \label{fig:mpst-rules}%
  %
\end{figure}


We explain each rule highlighting the new rules from
\cite{scalasLess2019}.
\begin{description}
  \item[Raise, promotion and prefixed processes]
    \inferrule{\iruleMPRaise} ensures that raise channel \chanraise
    only appears as a carried channel (like a constant) and never used
    as prefixes.

    \inferrule{\iruleMPPromote} says the try processes
    a part of typable processes; \inferrule{\iruleMPNil},
    \inferrule{\iruleMPBranch} and \inferrule{\iruleMPSel} are the standard rules for
    inaction, branching and selection but the
    derived conclusion ensures these processes can be placed in
    the try-position. Note that
    the premise
    $\stEnv$ in $\stJudge{\mpEnv}{%
        \stEnv \stEnvComp%
        \stEnvMap{y_i}{\stS[i]} \stEnvComp%
        \stEnvMap{\mpC}{\stSi[i]}%
      }{%
        \mpP[i]%
      }%
    $ in \inferrule{\iruleMPBranch} ensures that
    selecting one branch in $\inferrule{\iruleMPCBra}$ is
    sufficient for type soundness.
    \inferrule{\iruleMPPar} is the standard and the conclusion $\vdash$
    ensures that a try process does not contain parallel processes.

  \item[Affine selection/branching]
    Rules \inferrule{\iruleMPQBranch} and
    \inferrule{\iruleMPQSel} are identical to the linear case while
    they are not allowed to place in the try place.

  \item[Try-catch]
    \inferrule{\iruleMPTryCatch} is the main typing rule: a try process
    is inferred by $\mpFmt{\vDash}$-rules to ensure either
    a single branching/selection, inaction or recursion for a single
    branching/selection; a cancel process does not contain free recursive
    variables; and broadcast a cancellation.

  \item[Cancellation]
    \inferrule{\iruleMPCancel} (resp. \inferrule{\iruleMPKills}) types a
    cancel process (resp. a kill process) which appears
    during reductions: the cancellation of
    $\mpChanRole{\mpS}{\roleP}$ is broadcasting the cancellation
    to all processes which belong to session $\mpS$.

  \item[Recursions]
    \inferrule{\iruleMPDefTry} and \inferrule{\iruleMPCallTry}
    ensure that except the first argument $x_1$, instantiated channels
    are never used except as outputs in selection (their functions
    are similar with constants). This ensures that a recursion
    inferred by $\vDash$ are always either selection, branching or
    inaction. \inferrule{\iruleMPDef} and \inferrule{\iruleMPCall}
    are identical to those of~\cite{scalasLess2019}.

  \item[Restriction]
    Processes are initially typed projecting a global type by \inferrule{\iruleMPInit},
    while running processes are typed by \inferrule{\iruleMPSafeRes}
    (see the proof of Theorem~\ref{thm:subjectreduction}).
\end{description}

%\begin{example}[Typing \AMPST processes]
%\end{example}
\subsection{Properties of affine multiparty session types}
\label{sec:properties}
This subsection proves the main properties of \AMPST processes.
A typing context generated from a global type by reductions
is always safe.

\begin{lemma} {\rm (\cite[Lemma 5.9]{scalasLess2019})}\
\label{lem:globalsafety}
  If $  \stEnvi = \setenum{%
      \stEnvMap{\mpChanRole{\mpS}{\roleP}}{\gtProj{\gtG}{\roleP}}%
    }_{\roleP \in \gtRoles{\gtG}}$
  then $\stEnvSafeP{\stEnvi}$.
\end{lemma}
%\begin{proof}
%\end{proof}

Unlike linear-logic based typing systems
\cite{mostrousAffine2018,fowlerExceptional2019}, we do \emph{not}
assume a typing system is closed modulo
$\equiv$ -- instead, we prove it is closed under $\equiv$, including
tricky cases for kill and \CODE{try-catch} processes.
\inApp

\begin{restatable}[Subject Congruence]{THM}{thmMPSTSubectCongruence}\rm
  \label{thm:subjectcong}
  If $\stJudge{\mpEnv}{\stEnv}{\mpQ}$ and
  $\mpQ\!\equiv\! \mpP$, then
  we have
  $\stJudge{\mpEnv}{%
      \stEnv%
    }{%
      \mpP
    }%
  $.
\end{restatable}

Initial processes models a user-written Rust program -- it does not contain
any runtime, having the name restrictions at the top level.

\begin{restatable}[Initial processes]{DEF}{defMPSTInitial}\rm
  Process $\stJudge{}{}{\mpP}$
  typed without using \inferrule{\iruleMPSafeRes} is called
  an \emph{initial process}.
\end{restatable}

Starting from the initial process, by Lemma~\ref{lem:globalsafety} and
 Theorem~\ref{thm:subjectcong},
\AMPST processes satisfy the \emph{type soundness}. The proof can be
found in~\Cref{app:AMPST}.

\begin{restatable}[Subject Reduction]{THM}{thmMPSTSubectReduction}\rm
  \label{thm:subjectreduction}
  Suppose $\stJudge{}{}{\mpQ}$ is an initial process.
  Then for all $P$ such that $\mpQ\!\mpMoveStar\! \mpP$,
  if $\mpP \mpMove \mpPi$,
  then
  $\stJudge{}{}{\mpPi}$.%
\end{restatable}

We now define the key process properties -- \emph{deadlock-freedom}
and \emph{liveness}.

\begin{restatable}[Process properties]{DEF}{defMPSTProcessProperties}\rm
  \label{def:process-properties}%
  \label{def:process-term}%
  \label{def:process-nterm}%
  \label{def:process-df}%
  \label{def:process-liveness}%
  \label{def:process-strong-liveness}%
  $\mpP$ is \textbf{deadlock-free} %
  iff %
  $\mpP \!\mpMoveStar\! \mpNotMoveP{\mpPi}$ %
  implies %
  $\mpPi \!\equiv\! \mpNil$.
  %
  %  \;$\mpP$ is \textbf{terminating} %
  %  iff %
  %  it is deadlock-free, %
  %  and %
  %  $\exists j$ finite such that, %
  %  $\forall n \!\ge\! j$, %
  %  $\mpP \!=\! \mpP[0] \!\mpMove\! \mpP[1] \!\mpMove\!%
  %  \dots \!\mpMove\! \mpP[n]$ %
  %  implies
  %  $\mpP[n] \!\equiv\! \mpNil$.
  %  %
  %  \;$\mpP$ is \textbf{never-terminating} %
  %  iff %
  %  $\mpP \!\mpMoveStar\! \mpPi$ %
  %  implies %
  %  $\mpMoveP{\mpPi}$.
  %  %
  \;$\mpP$ is \textbf{live} %
  iff %
  $\mpP \!\mpMoveStar\! \mpPi \!\equiv\! \mpCtxApp{\mpCtx}{\mpQ}$ \,implies:
  \begin{enumerate}%[leftmargin=1em]
    \item\label{item:process-liveness:sel}%
    if\; %
    $\mpQ = \mpSel{\mpC}{\roleQ}{\mpLab}{\mpChanRole{\mpSi}{\roleR}}{\mpQi}$ %
    (for some $\mpLab, \mpSi, \roleR, \mpQi$), %
    \;then\; %
    $\exists \mpCtxi$: %
    $\mpPi \!\mpMoveStar\! \mpCtxApp{\mpCtxi}{\mpQi}$; %
    \;and
    \item\label{item:process-liveness:branch}%
    if\; %
    $\mpQ = \mpBranch{\mpC}{\roleQ}{i \in I}{\mpLab[i]}{x_i}{\mpQi[i]}$ %
    (for some $\mpLab[i], \mpFmt{x_i}, \mpQi[i]$), % for $i \!\in\! I$)
    \;then\; %
    $\exists \mpCtxi, k \!\in\! I, \mpSi, \roleR$:\, %
    $\mpPi \!\mpMoveStar\! \mpCtxApp{\mpCtxi}{\mpQi[k]\subst{x_k}{\mpChanRole{\mpSi}{\roleR}}}$.%
  \end{enumerate}
  %  %
  %  $\mpP$ is \textbf{strongly live} iff\, %
  %  $\mpP \!\mpMoveStar\! \mpPi \!\equiv\! \mpCtxApp{\mpCtx}{\mpQ}$ \,implies:
  %  \begin{enumerate}[resume]%[leftmargin=1em]
  %  \item\label{item:process-strong-liveness:sel}%
  %    item~\ref{item:process-liveness:sel} above, %
  %    and moreover, %
  %    there is $n$ finite %
  %    such that, whenever %
  %    $\mpPi = \mpPi[0] \mpMove \mpPi[1] \mpMove%
  %    \dots \mpMove \mpPi[n]$, %
  %    then for some $j \!\le\! n$ we have %
  %    $\mpPi[j] \!\mpMove\! \mpCtxApp{\mpCtxii}{\mpQi}$ %
  %    (for some $\mpCtxii$);%
  %  \item\label{item:process-strong-liveness:branch}%
  %    item~\ref{item:process-liveness:branch} above, %
  %    and moreover, %
  %    there is $n$ finite %
  %    such that, whenever %
  %    $\mpPi = \mpPi[0] \mpMove \mpPi[1] \mpMove%
  %    \dots \mpMove \mpPi[n]$, %
  %    then for some $j \!\le\! n$ we have %
  %    $\mpPi[j] \!\mpMove\!%
  %    \mpCtxApp{\mpCtxii}{\mpQi[k]\subst{x_k}{\mpChanRole{\mpSi}{\roleR}}}$
  %    (for some $\mpCtxii, k \!\in\! I, \mpSi, \roleR$).%
  %  \end{enumerate}
\end{restatable}

A single agent in a multiparty session $s$ is a
participant playing a single role $\roleP$ in $s$.

\begin{DEF}[An agent with a unique role in a session (\cite{scalasLess2019})]
  \label{def:unique-role-proc}%
  Assume\; $\stJudge{\mpEnvEmpty}{\stEnv}{\mpP}$.
  \;We say that $\mpP$:
  \begin{enumerate}[leftmargin=4mm]%
    \item\label{item:guarded-definitions:stmt}%
    \textbf{has guarded definitions} %
    \;iff\; %
    in each subterm of the form\, %
    $\mpDef{\mpX}{\stEnvMap{x_1}{\stS[1]},...,\stEnvMap{x_n}{\stS[n]}}{
        \mpQ}{\mpPi}$, %
    % $n \ge 1$ \,and\, %
    \,for all $i \in 1..n$,\, %
    $\stS[i] \!\stNotSub\! \stEnd$ %
    \,implies\, %
    that a call $\mpCall{\mpY}{...,x_i,...}$ %
    can only occur in $\mpQ$ %
    as subterm of\; %
    $\mpBranch{x_i}{\roleQ}{j \in J}{\mpLab[j]}{y_j}{\mpP[j]}$ %
    \,or\, %
    $\mpSel{x_i}{\roleQ}{\mpLab}{\mpC}{\mpPii}$ %
    (\ie after using $x_i$ for input/output);%
    \item\label{item:unique-role-proc:stmt}
    \textbf{only plays role $\roleP$ in $\mpS$, by $\stEnv$\!,} %
    \,iff:\; %
    \begin{enumerate}[ref=\emph{(\roman*)},label=\emph{(\roman*)}]
      \item%
      $\mpP$ has guarded definitions;\; % (by $\stEnv$), %
      \item%
      $\fv{\mpP} \!=\! \emptyset$;\; %
      \item\label{item:unique-role-proc:stenv}%
      $\stEnv \!=\!%
        \stEnv[0] \stEnvComp \stEnvMap{\mpChanRole{\mpS}{\roleP}}{\stS}$
      with %
      $\stS \!\stNotSub\! \stEnd$ %
      and %
      $\stEnvEndP{\stEnv[0]}$;\; %
      \item\label{item:unique-role-proc:res-end}%
      in all subterms %
      $\mpRes{\stEnvMap{\mpSi}{\stEnvi}}{\mpPi}$ %
      of $\mpP$, %
      we have $\stEnvEndP{\stEnvi}$.
    \end{enumerate}
  \end{enumerate}
  %
  We say ``\textbf{$\mpP$ only plays role $\roleP$ in $\mpS$}'' %
  \,iff\, %
  $\exists\stEnv: \stJudge{\mpEnvEmpty\!}{\!\stEnv\!}{\!\mpP}$, %
  and item~\ref{item:unique-role-proc:stmt} holds.
\end{DEF}

The advantage of \AMPST is \emph{no change of global and local types}:
Taking a kill process into account, \emph{session fidelity} is derived
directly from one in~\cite{scalasLess2019}.

\begin{restatable}[Session Fidelity (\cite{scalasLess2019})]{THM}{lemSessionFidelity}%
  \label{lem:session-fidelity}%
  Assume\, $\stJudge{\mpEnvEmpty\!}{\!\stEnv}{\!\mpP}$, %
  where %
  $\stEnv$ is safe, %
  \,$\mpP \equiv \mpBigPar{\roleP \in I}{\mpP[\roleP]}$, %
  \,and\, $\stEnv = \bigcup_{\roleP \in I}\stEnv[\roleP]$
  %  \fxASwarning{Here we use $\cup$ because $\stEnv$ is a partial mapping
  %    (hence a set of pairs), but this might not be obviously clear}%
  % with $\bigcap_{\roleP \in I}\stEnv[\roleP] = \stEnvEmpty$;
  % further,
  such that, for each $\mpP[\roleP]$, %
  we have\, $\stJudge{\mpEnvEmpty\!}{\stEnv[\roleP]}{\!\mpP[\roleP]}$;
  \,further, assume that each $\mpP[\roleP]$
  is either\, $\mpNil$ (up-to $\equiv$), %
  or only plays $\roleP$ in $\mpS$, by $\stEnv[\roleP]$.
  Then, %
  $\stEnvMoveP{\stEnv}$ %
  \,implies\; %
  $\exists \stEnvi,\mpPi$ %
  such that\, %
  $\stEnv \!\stEnvMove\! \stEnvi$, %
  $\mpP \!\mpMoveStar\! \mpPi$ %
  \,and\, %
  $\stJudge{\mpEnvEmpty\!}{\!\stEnvi}{\mpPi}$, %
  \;with\; %
  $\stEnvi$ safe, %
  \,$\mpPi \equiv \mpBigPar{\roleP \in I}{\mpPi[\roleP]}$, %
  \,and\, $\stEnvi = \bigcup_{\roleP \in I}\stEnvi[\roleP]$
  such that, for each $\mpPi[\roleP]$, %
  we have\, $\stJudge{\mpEnvEmpty\!}{\stEnvi[\roleP]}{\!\mpPi[\roleP]}$,
  \,and each $\mpPi[\roleP]$
  is either\, $\mpNil$, %
  $\kills{\mpS}$,
  or only plays $\roleP$ in $\mpS$, by $\stEnvi[\roleP]$.%
\end{restatable}


Now we consider more than two parallel composed threads
which are spawned by a user-written Rust program with one session.

\begin{DEF}[Initial multiparty session]\label{def:initialsingle}
  \label{def:imps}%
  \rm
  We say
  $\stJudge{}{}{\mpQ}$ is an \emph{initial multiparty session process} if
  $\mpQ \equiv \mpRes{\stEnvMap{\mpS}{\stEnv}}{\mpBigPar{\roleP \in \gtG}{\mpP[\roleP]}}$,
  $\mpP[\roleP]$ only plays $\roleP$ in $\mpS$,
  and $\stEnv = \setenum{\stEnvMap{\mpChanRole{\mpS}{\roleP}}{\gtProj{\gtG}{\roleP}}}_{\roleP \in \gtG},\stEnv'$
  for some $\gtG$ and $\stEnvEndP{\stEnv'}$.
\end{DEF}


Now we state the three main theorems of this paper: deadlock-freedom
and liveness, and cancellation termination properties.
The cancellation termination theorem states that
once a cancellation is triggered by one of the multi-threaded processes,
or an affine channel is waiting forever (due to a timeout or an
error), then all processes will eventually terminate.

\begin{THM}[\cite{scalasLess2019}]
  \label{lem:process-df-live-from-ctx}%
  Assume\; $\stJudge{\mpEnvEmpty}{\stEnv}{\mpP}$,
  \;with $\stEnv$ safe,\;
  $\mpP \equiv \mpBigPar{\roleP \in I}{\mpP[\roleP]}$,
  each $\mpP[\roleP]$ %
  having guarded definitions %
  and either being $\mpNil$ (up-to $\equiv$),
  or only playing role $\roleP$ in $\mpS$.
  \;Then,\; %
  \begin{enumerate}[label=(\arabic*)]
    \item\label{item:process-df-live-from-ctx:df}%
    \,$\stEnvDFP{\stEnv}$
    implies that %
    $\mpP$ is deadlock-free; and
    \item\label{item:process-df-live-from-ctx:live}%
    \,$\stEnvLivePlusP{\stEnv}$ %
    % \,or\, %
    % $\stEnvProjP{\gtG}{\mpS}{\stEnv}$ (for some $\gtG$) %
    implies that %
    $\mpP$ is live.
  \end{enumerate}
\end{THM}

\begin{restatable}[]{COL}{colDeadlockFree}\rm
  \label{cor:liveness}
  Suppose $\stJudge{}{}{\mpQ}$ is an initial multiparty session
  process.
  % is an initial and guarded multiparty session process,
  % typed by $n=1$ in \inferrule{\iruleMPInit},
  Then for all $P$ such that $\mpQ\!\mpMoveStar\! \mpP$, $\mpP$
  is deadlock-free and live.
\end{restatable}
\begin{proof}
  If $Q$ is a single initial multiparty session process, then
  we can write: $Q =\mpRes{\stEnvMap{\mpS}{\stEnv}}{\mpR}$
  with $\mpR= \mpBigPar{\roleP \in I}{\mpR[\roleP]}$
  and each $\mpP[\roleP]$ %
  either is\, $\mpNil$ (up-to $\equiv$), %
  or only plays $\roleP$ in $\mpS$.
  The rest is by Theorems~\ref{lem:session-fidelity}
  and~\ref{lem:process-df-live-from-ctx}. See
  Remark 5.12 in~\cite{scalasLess2019}.
\end{proof}

\begin{restatable}[Cancellation Termination]{THM}{thm:CancellationTermination}\
  \label{thm:ctermination}%
  Suppose $\stJudge{}{}{\mpQ}$ is an initial multiparty session
  process.
  \begin{enumerate}
    \item If $\mpQ\!\mpMoveStar\!
            \mpCtx{}{[{\mpCancel{\mpChanRole{\mpS}{\roleP}}{\mpQ'}}]}=\mpP'$,
          then we have $\mpP'\mpMoveStar\mpNil$.
    \item
          If $\mpQ\!\mpMoveStar\!
            \mpCtx{}{[
                  \mpQuestionBranch{\mpChanRole{\mpS}{\roleP}}{\roleQ}{i \in I}{%
                    \mpLab[i]}{x_i}{\mpP[i]}]}=\mpP'$ or
          $\mpQ\!\mpMoveStar\! \mpCtx{}{[
                  \mpQuestionSel{\mpChanRole{\mpS}{\roleP}}{\roleQ}{\mpLab}{
                    \mpChanRole{\mpS'}{\roleR}}{\mpP}]}=\mpP'$
          with
          $\mpP' \equiv \mpRes{\stEnvMap{\mpS}{\stEnv}}{\mpR}$ and
          $\mpChanRole{\mpS}{\roleQ}\not\in \fc{\mpR}$,
          then we have $\mpP'\mpMoveStar\mpNil$.
  \end{enumerate}
\end{restatable}
\begin{proof}
  (1) By \inferrule{\iruleMPTryCatch}, $\fpv{\mpQ'}=\emptyset$;
  and by Definition~\ref{def:imps} (and the conditions of Definition~\ref{def:unique-role-proc}),
  $\mpQ'$ does not contain
  any branching/selection (under restrictions) except whose subject is
  $s$. Hence $\mpCtx{}{[\mpQ'\mpPar \kills{s}]}\mpMoveStar
    \mpRes{s}{(\kills{s}\mpPar \dots \mpPar \kills{s})}\equiv \mpNil$,
  as desired. (2)
  Assume $\mpQ\!\mpMoveStar\!
    \mpCtx{}{[
          \mpQuestionBranch{\mpChanRole{\mpS}{\roleP}}{\roleQ}{i \in I}{%
            \mpLab[i]}{x_i}{\mpP[i]}]}=\mpP'$.
  If $\mpChanRole{\mpS}{\roleQ}\not\in \fc{\mpP'}$,
  by Corollary~\ref{cor:liveness},
  there exists no $\mpP''$ such that
  $\mpP'\!\mpMoveStar\! \mpCtx{}{[
          \mpQuestionSel{\mpChanRole{\mpS}{\roleQ}}{\roleP}{\mpLab}{
            \mpChanRole{\mpS'}{\roleR}}{\mpP}]}=\mpP''$.
  Hence it triggers the exception at $s$ in $\inferrule{\iruleMPCQBra}$.
  The rest is similar with (1). The case for the affine selection is the
  same.
\end{proof}




==> plan.tex <==
\section{Future work}
\label{sec:futureWork}

% I submitted my ideas for implementing Multiparty Session Types in Rust at the workshop PLACES 2020, and the related paper was accepted.
% I published my current implementation at the conference COORDINATION 2020~\cite{bliudzeimplementing2020}.
% I intend to continue on this path and work on my tool,~\mpstrust.
% I divided my future work into two parts, achieved in parallel: a theoretical and a practical one.
% The latter is focused on the implementation of features and the evaluation of the tool, while the former is focused on the formalisation of our tool.
% The writing of my thesis follows those milestones.
% The timetable of the project can be found below in~\Cref{tab:timetable}.
% This timetable is divided in three columns, where the first one contains the deadlines for the different tasks, the two others describe the practical and theoretical activities, in chronological order, from top to bottom.
%
%\begin{table}[t!]
%	\centering
%	\begin{tabular}{c | c |c }
%		Time & Practical activities & Theoretical activities \\
%		\hline\hline
%		12 July 2020 & \multicolumn{2}{c}{ESR} \\
%		\hline
%		October 2020 & \makecell{Parametrisation of\\the number and name\\of participants} & Based on~\cite{castrodistributed2019, fowler2019exceptional} \\
%		\hline
%		December 2020 & \emph{Linter} for~\mpstrust & N/A \\
%		\hline
%		March 2021 & Evaluation of~\mpstrust & \makecell{Formalisation:\\MPST for affine channels} \\
%		\hline
%		June 2021 & Inference of protocols & \makecell{Formalisation:\\choreography protocol synthesis} \\
%		\hline
%		2022 & \multicolumn{2}{c}{Writing up thesis} \\
%		\hline
%		May 2022 & \multicolumn{2}{c}{Submitting examination entry} \\
%		\hline
%		September 2022 & \multicolumn{2}{c}{Submitting thesis} \\
%	\end{tabular}
%	\caption{Timetable}
%	\label{tab:timetable}
%\end{table}
%
% One practical step will be the implementation of various features for generalising the possibilities of~\mpstrust.
% This process includes the parametrisation of my tool on the number of participants, the name of the roles and the number of sessions.
% Indeed, my current library can only handle Multiparty Session Types for 3 participants, but most of the real protocols involve more participants.
Our library can handle most real life situations, but it remains incomplete on a practical and theoretical basis.
In most of the protocols, not all participants communicate with all others: some may form a peninsula and having to define the binary session types between them and another peninsula of participants will make the protocol burdensome.
Hence, being able to create a Rust \CODE{struct} for types that are parametrised on the number of participants and sessions is crucial.
% Removing the limitation on the names of the roles is another key feature: currently, the only available roles are \role{A}, \role{B} and \role{C}.
Another useful feature would be the implementation of a \emph{linter}, a plugin for the Rust compiler, to check more errors at compile-time and return human-readable and effective tooltips.
Currently, our tool returns the full expected types and the types that were found when an error is detected, and not the exact faulty part of a wrong type, which is not very user-friendly.
% That is why the implementation of those features would be welcomed by current and future users.
% During this chapter, we will also investigate the optimisation opportunities based on protocol analysis.
% Indeed, the main difference with code-generation of our approach and existing ones is that we generate.
Another step is the \emph{formalisation} of~\mpstrust: we need to define to what extent~\mpstrust follows the usual requirements of specific theories.
This process includes the verification of safety and liveness, the limitations and the strengths and the description of our implementation of affine types.
Indeed, Rust uses affine types rather than linear types, and the work done on this language may help to implement \MPST on other languages with such types.
This process also includes \emph{automata synthesis}: being able to translate our protocols into choreography automata will add a layer of credibility to our tool.
\emph{Automata synthesis} is a more mature theory than session types (section~\ref{subsec:automatas}), that can describe interactions between participants too, but does not rely on syntax.
For our project, this means that we have to be able to extract automata from our protocols, automata that can then be checked by state-of-the-art tools.
The \emph{evaluation} of our tool and \emph{inference of protocols} are another practical step before the writing of the thesis.
\emph{Protocols} inference is the code-generation of types from snippets of code.
The \emph{evaluation} comes from the fact that \MPST is intended to be used for many participants, thus,~\mpstrust has to be tested close to real-life situations, at large scale.
The measured metrics will include the performances, the number of maximum participants that can be handled, the correlation between the number of participants and the complexity of the protocols, and the compile time.
This may lead to refactor our tool in order to increase the performances and the scaling.
Benchmarks will be set up around curating protocols, from existing ones or new ones specially created for~\mpstrust.

%call-back/non call-back > benchmark > check integrity
%
%affine
%
%practical > formalism > extension (parametric)

==> theory/Makefile <==
NAME=main

TEX=$(NAME).tex
PDF=$(NAME).pdf

TEXOPTS=

CLEAN=*.aux *.log *.dvi *.toc *.out *.vtc *.cfg *.glo *.idx *.ilg *.ind *.lof *.lot *.gls *.cut *.hd *.ps *.thm *.rpi *.cut *.upa *.blg *.ptc figure/*.xbb

all: pdf

pdf:
	pdflatex $(TEXOPTS) $(TEX)
	bibtex $(NAME) || true
	pdflatex $(TEXOPTS) $(TEX)
	pdflatex $(TEXOPTS) $(TEX)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' main.log) \
	do pdflatex $(TEXOPTS) $(TEX); done

fastpdf:
	pdflatex $(TEXOPTS) $(TEX)
	open -a Skim.app $(PDF)


clean:
	rm -f $(CLEAN)
	cd artifact
	rm -f $(CLEAN)

distclean: clean
	rm -f *.pdf *.bbl

TECHREPORT_DIR=techreport-$(shell git rev-parse --short HEAD)
CAMERAREADY_DIR=cameraready-$(shell git rev-parse --short HEAD)
ARTIFACT_DIR=artifact-$(shell git rev-parse --short HEAD)

techreport-zip:
	rm -rf $(TECHREPORT_DIR) $(TECHREPORT_DIR).zip techreport.tex
	latexpand --empty-comments main.tex >techreport.tex
	mkdir $(TECHREPORT_DIR)
	cp techreport.tex lipics-v2019.cls session.bib orcid.pdf $(TECHREPORT_DIR)
	mkdir $(TECHREPORT_DIR)/figures; mkdir $(TECHREPORT_DIR)/Graphs
	cp figures/*.png  $(TECHREPORT_DIR)/figures
	cp figures/*.pdf  $(TECHREPORT_DIR)/figures
	cp Graphs/*.pdf  $(TECHREPORT_DIR)/Graphs
	find $(TECHREPORT_DIR) -type f -exec chmod -w {} \;
	cd $(TECHREPORT_DIR); pdflatex $(TEXOPTS) techreport.tex; bibtex techreport; rm -f $(CLEAN) techreport.pdf
	zip -r $(TECHREPORT_DIR).zip $(TECHREPORT_DIR)

cameraready-zip:
	rm -rf $(CAMERAREADY_DIR) $(CAMERAREADY_DIR).zip
	mkdir $(CAMERAREADY_DIR)
	cp Makefile *.tex lipics-v2019.cls session.bib orcid.pdf $(CAMERAREADY_DIR)
	cp -r section $(CAMERAREADY_DIR)
	mkdir $(CAMERAREADY_DIR)/figures; mkdir $(CAMERAREADY_DIR)/Graphs
	cp figures/*.png  $(CAMERAREADY_DIR)/figures
	cp figures/*.pdf  $(CAMERAREADY_DIR)/figures
	cp Graphs/*.pdf  $(CAMERAREADY_DIR)/Graphs
	find $(CAMERAREADY_DIR) -type f -exec chmod -w {} \;
	make -C $(CAMERAREADY_DIR)
	zip -r $(CAMERAREADY_DIR).zip $(CAMERAREADY_DIR)

artifact-zip:
	rm -rf $(ARTIFACT_DIR) $(ARTIFACT_DIR).zip
	mkdir $(ARTIFACT_DIR)
	cp artifact/main.tex artifact/*.cls artifact/darts-logo-bw.pdf artifact/lipics-logo-bw.pdf artifact/orcid.pdf artifact/cc-by.pdf $(ARTIFACT_DIR)
	find $(ARTIFACT_DIR) -type f -exec chmod -w {} \;
	cd $(ARTIFACT_DIR); pdflatex main
	zip -r $(ARTIFACT_DIR).zip $(ARTIFACT_DIR)


==> theory/extra_packages.tex <==
\usepackage{thm-restate}
\usepackage{amsfonts}
\usepackage{cleveref}
\usepackage[page,header]{appendix}
\usepackage{titletoc}
\usepackage{setspace}
\usepackage{enumitem}
\usepackage{wrapfig}
\usepackage[framemethod=TikZ]{mdframed}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc} %support umlauts in the input
\usepackage{subcaption}
\captionsetup{compatibility=false}

\usepackage{etoolbox}
\usepackage{xifthen}
\usepackage{xspace}
\usepackage{thmtools}
\usepackage{thm-restate}

%
% Enable correct jumping to figures when referencing
\usepackage[all]{hypcap}
\usepackage{nicefrac}
% show back-tick symbol ` correctly as the original one would be confused with '
\usepackage{upquote}

% \llbracket, \rrbracket
\usepackage{stmaryrd}
% fix: warning ``LaTeX Font Warning: Font shape `U/stmry/b/n' undefined''
% https://tex.stackexchange.com/questions/106714/stmaryrd-and-boldsymbol-avoid-warnings
\SetSymbolFont{stmry}{bold}{U}{stmry}{m}{n}
% fix: Font shape `U/stmry/m/n' in size <5.5> not available (Font) size <5> substituted on input line
\usepackage{anyfontsize}

% \llangle, \rrangle
% \usepackage{MnSymbol}

\usepackage{proof}
\usepackage{mathtools} % for \mathrlap{}
\usepackage{mathrsfs}
\usepackage[most]{tcolorbox}
\usepackage{xcolor}
\usepackage{graphicx,graphics}
\usepackage{url}
\usepackage{color}
\usepackage{comment}
\usepackage{rotating}
\usepackage{listings}
\usepackage{multicol}
\usepackage{multirow}
\usepackage[noend]{algpseudocode}
\usepackage{tikz}
\usepackage{fancybox}
\usetikzlibrary{positioning,calc,backgrounds,fit,shapes,arrows.meta,cd}
\usepackage{import}
\usepackage{makecell}
\usepackage{relsize}
\usepackage{listings}

% For easy quotations: \enquote{text}
% This package is very smart when nesting is applied, otherwise textcmds (see below) provides a shorter command
\usepackage{csquotes}

% Nicer tables (\toprule, \midrule, \bottomrule)
\usepackage{booktabs}

% \usepackage[group-four-digits,per-mode=fraction]{siunitx}
\usepackage[group-minimum-digits=4,per-mode=fraction]{siunitx}
% Check https://texnique.fr/osqa/questions/10133/mise-a-jour-problematique-du-package-siunitx
% may replace group-minimum-digits=4 with group-four-digits

\usepackage{adjustbox} % for resizing tables
\usepackage{arydshln} % dashed \hline

% Enable nice comments
% XXX LOAD THIS AS THE LAST PACKAGE (hyperref restriction)
\usepackage{pdfcomment}

% Enable that parameters of \cref{}, \ref{}, \cite{}, ...
%are linked so that a reader can click on the number an jump to the target in the document
% \usepackage{hyperref} % loaded by pdfcomment package above
\hypersetup{hidelinks,
  unicode,
  colorlinks=true,
  allcolors=black,
  pdfstartview=Fit,
  breaklinks=true}

%improve wrapping of URLs - hint by http://tex.stackexchange.com/a/10419/9075
\makeatletter
\g@addto@macro{\UrlBreaks}{\UrlOrds}
\makeatother

% Prepare more space-saving rendering of the bibliography
% Source: https://tex.stackexchange.com/a/280936/9075
\SetExpansion
  [ context = sloppy,
    stretch = 30,
    shrink = 60,
    step = 5 ]
  { encoding = {OT1,T1,TS1} }
  { }

% Intermediate solution for hyperlinked refs.
% See https://tex.stackexchange.com/q/132420/9075 for more information.
\newcommand{\Vlabel}[1]{\label[line]{#1}\hypertarget{#1}{}}
\newcommand{\lref}[1]{\hyperlink{#1}{\FancyVerbLineautorefname~\ref*{#1}}}
